Advances in Global Solvers for 3D Vision

Global solvers have emerged as a powerful paradigm for 3D vision, offering certifiable solutions to nonconvex geometric optimization problems traditionally addressed by local or heuristic methods. This survey presents the first systematic review of global solvers in geometric vision, unifying the field through a comprehensive taxonomy of three core paradigms: Branch-and-Bound (BnB), Convex Relaxation (CR), and Graduated Non-Convexity (GNC). We present their theoretical foundations, algorithmic designs, and practical enhancements for robustness and scalability, examining how each addresses the fundamental nonconvexity of geometric estimation problems. Our analysis spans ten core vision tasks, from Wahba problem to bundle adjustment, revealing the optimality-robustness-scalability trade-offs that govern solver selection. We identify critical future directions: scaling algorithms while maintaining guarantees, integrating data-driven priors with certifiable optimization, establishing standardized benchmarks, and addressing societal implications for safety-critical deployment. By consolidating theoretical foundations, practical advances, and broader impacts, this survey provides a unified perspective and roadmap toward certifiable, trustworthy perception for real-world applications. A continuously-updated literature summary and companion code tutorials are available at https://github.com/ericzzj1989/Awesome-Global-Solvers-for-3D-Vision.

==> fig/tasks/ba_data.tex <==
% Camera positions
\coordinate (O1) at (-7.666, -7.452, -14.655);
\coordinate (O2) at (0.281, -7.211, -15.618);
\coordinate (O3) at (7.504, -6.970, -14.173);

% 3D points
\coordinate (X0) at (-1.635, 0.541, 1.193);
\coordinate (X1) at (-0.383, -0.300, -1.641);
\coordinate (X2) at (-3.477, 0.342, 0.509);
\coordinate (X3) at (0.898, -0.380, -1.587);
\coordinate (X4) at (-2.741, -0.240, 0.190);
\coordinate (X5) at (-1.314, -0.330, 0.619);
\coordinate (X6) at (-2.948, -0.259, -0.580);
\coordinate (X7) at (-1.239, 0.295, -1.504);
\coordinate (X8) at (-0.971, 0.074, -2.160);
\coordinate (X9) at (-0.331, -0.390, -2.090);
\coordinate (X10) at (-2.101, -0.290, 0.836);
\coordinate (X11) at (-1.234, -0.266, 0.045);
\coordinate (X12) at (-3.629, 0.369, -1.053);
\coordinate (X13) at (-0.087, -0.239, 0.101);
\coordinate (X14) at (-0.287, 0.320, -1.832);
\coordinate (X15) at (-2.620, -0.346, -0.841);
\coordinate (X16) at (-1.716, -0.105, 0.159);
\coordinate (X17) at (-3.025, 0.293, -2.116);
\coordinate (X18) at (1.933, 0.223, -1.432);
\coordinate (X19) at (-3.814, 0.260, 1.029);
\coordinate (X20) at (0.385, 0.247, -2.070);
\coordinate (X21) at (-0.139, -0.250, -2.057);
\coordinate (X22) at (-2.095, -0.262, 1.086);
\coordinate (X23) at (-0.042, 0.454, -0.083);
\coordinate (X24) at (-0.557, 0.141, -0.061);
\coordinate (X25) at (-0.797, -0.018, -2.411);
\coordinate (X26) at (-3.201, -0.428, 0.752);
\coordinate (X27) at (-2.390, -0.343, -0.948);
\coordinate (X28) at (-2.758, 0.487, 0.121);
\coordinate (X29) at (0.896, 0.341, -0.945);
\coordinate (X30) at (-3.161, -0.176, -0.379);
\coordinate (X31) at (0.806, 0.354, -2.347);
\coordinate (X32) at (-0.822, 0.002, -1.309);
\coordinate (X33) at (-2.061, 0.012, 0.987);
\coordinate (X34) at (-2.345, 0.059, -0.815);
\coordinate (X35) at (-2.103, -0.378, 0.565);
\coordinate (X36) at (-0.880, -0.329, -1.129);
\coordinate (X37) at (1.411, -0.294, -1.649);
\coordinate (X38) at (-0.895, 0.437, -1.381);
\coordinate (X39) at (0.042, 0.331, -1.191);
\coordinate (X40) at (0.426, -0.135, 0.578);
\coordinate (X41) at (-0.114, -0.013, -1.782);
\coordinate (X42) at (1.056, -0.202, -1.520);
\coordinate (X43) at (-3.584, 0.083, 0.969);
\coordinate (X44) at (-3.704, -0.028, -1.147);
\coordinate (X45) at (-0.081, -0.245, 0.909);
\coordinate (X46) at (-1.552, 0.456, -1.849);
\coordinate (X47) at (1.178, -0.195, 0.810);
\coordinate (X48) at (0.936, 0.080, 0.213);
\coordinate (X49) at (1.489, 0.260, -0.514);
\coordinate (X50) at (1.354, 0.243, 0.856);
\coordinate (X51) at (-0.451, -0.406, -2.035);
\coordinate (X52) at (0.024, -0.614, -1.623);
\coordinate (X53) at (-0.523, 0.224, 0.703);
\coordinate (X54) at (-2.519, 0.218, -1.198);
\coordinate (X55) at (-2.031, 0.293, 0.559);
\coordinate (X56) at (1.049, 0.129, 0.408);
\coordinate (X57) at (-3.270, -0.216, -1.168);
\coordinate (X58) at (-2.388, 0.463, -0.523);
\coordinate (X59) at (-0.914, 0.244, -0.105);
\coordinate (X60) at (-2.818, 0.284, -1.071);
\coordinate (X61) at (-3.695, 0.096, -1.540);
\coordinate (X62) at (1.101, -0.187, -0.570);
\coordinate (X63) at (1.121, -0.108, -1.675);
\coordinate (X64) at (-0.573, 0.500, 0.948);
\coordinate (X65) at (-0.468, -0.172, 0.580);
\coordinate (X66) at (1.937, -0.387, 0.135);
\coordinate (X67) at (1.291, 0.259, 0.909);
\coordinate (X68) at (0.262, -0.017, -0.928);
\coordinate (X69) at (1.485, -0.045, 0.064);
\coordinate (X70) at (0.729, 0.112, 1.020);
\coordinate (X71) at (0.808, 0.303, -0.671);
\coordinate (X72) at (-1.601, -0.429, 0.299);
\coordinate (X73) at (-3.616, -0.053, 0.247);
\coordinate (X74) at (-2.183, -0.045, -2.256);
\coordinate (X75) at (-3.619, 0.369, -0.690);
\coordinate (X76) at (-2.582, 0.193, -1.958);
\coordinate (X77) at (-3.432, 0.015, 0.150);
\coordinate (X78) at (-2.290, -0.056, -1.991);
\coordinate (X79) at (0.273, -0.079, -1.522);
\coordinate (X80) at (-2.930, -0.130, 0.256);
\coordinate (X81) at (0.334, 0.250, -1.082);
\coordinate (X82) at (1.818, 0.131, 0.413);
\coordinate (X83) at (-0.305, -0.082, -1.318);
\coordinate (X84) at (-1.789, 0.186, -2.349);
\coordinate (X85) at (-3.152, -0.355, -2.163);
\coordinate (X86) at (1.153, 0.130, -0.154);
\coordinate (X87) at (-3.118, -0.048, 0.025);
\coordinate (X88) at (-2.829, -0.051, -0.378);
\coordinate (X89) at (-0.162, 0.135, -2.184);
\coordinate (X90) at (-1.652, 0.158, 0.113);
\coordinate (X91) at (1.137, 0.210, -1.471);
\coordinate (X92) at (-3.377, 0.172, -2.356);
\coordinate (X93) at (-0.618, 0.465, 0.390);
\coordinate (X94) at (-1.607, 0.168, -0.172);
\coordinate (X95) at (-0.578, 0.444, -0.569);
\coordinate (X96) at (1.813, 0.388, -1.393);
\coordinate (X97) at (-3.446, -0.419, -2.281);
\coordinate (X98) at (-3.266, 0.224, -2.051);
\coordinate (X99) at (-2.102, 0.314, -2.205);
\coordinate (X100) at (0.872, -0.215, -1.734);
\coordinate (X101) at (0.400, 0.235, -1.029);
\coordinate (X102) at (2.042, -0.096, -0.563);
\coordinate (X103) at (-0.864, 0.346, -0.740);
\coordinate (X104) at (1.187, -0.266, -2.358);
\coordinate (X105) at (1.499, -0.494, -1.054);
\coordinate (X106) at (1.719, 0.464, 0.308);
\coordinate (X107) at (-0.233, -0.107, -0.954);
\coordinate (X108) at (-1.959, 0.215, 1.043);
\coordinate (X109) at (0.700, 0.210, -1.954);
\coordinate (X110) at (-0.994, -0.356, 0.138);
\coordinate (X111) at (-1.258, 0.427, -0.550);
\coordinate (X112) at (-3.171, -0.308, 1.163);
\coordinate (X113) at (-0.413, -0.310, -1.970);
\coordinate (X114) at (0.404, -0.360, -1.946);
\coordinate (X115) at (1.890, -0.222, -0.492);
\coordinate (X116) at (0.456, -0.003, -1.997);
\coordinate (X117) at (0.783, 0.063, -0.464);
\coordinate (X118) at (1.489, -0.404, 0.048);
\coordinate (X119) at (-3.745, -0.129, -2.091);
\coordinate (X120) at (-2.968, -0.320, 0.748);
\coordinate (X121) at (-2.581, 0.562, -2.323);
\coordinate (X122) at (-0.708, 0.467, -2.023);
\coordinate (X123) at (-0.576, 0.486, 0.001);
\coordinate (X124) at (-0.257, 0.268, -0.195);
\coordinate (X125) at (1.262, -0.035, 0.638);
\coordinate (X126) at (-2.059, -0.397, -0.058);
\coordinate (X127) at (-1.701, 0.037, -1.985);
\coordinate (X128) at (1.785, 0.495, 1.097);
\coordinate (X129) at (0.830, 0.370, 1.130);
\coordinate (X130) at (1.093, -0.496, -2.197);
\coordinate (X131) at (-2.891, 0.089, -0.574);
\coordinate (X132) at (-1.077, -0.099, -0.985);
\coordinate (X133) at (1.940, 0.490, 0.293);
\coordinate (X134) at (-2.309, -0.078, -1.687);
\coordinate (X135) at (1.823, 0.086, -1.224);
\coordinate (X136) at (-0.014, 0.181, -0.635);
\coordinate (X137) at (-3.122, 0.131, 0.011);
\coordinate (X138) at (-1.407, -0.387, -2.234);
\coordinate (X139) at (0.548, 0.014, 0.948);
\coordinate (X140) at (-2.623, -0.485, -2.301);
\coordinate (X141) at (-1.805, -0.021, -0.456);
\coordinate (X142) at (-1.233, 0.418, -0.721);
\coordinate (X143) at (-0.800, 0.335, -0.443);
\coordinate (X144) at (-3.006, 0.575, -0.042);
\coordinate (X145) at (-1.092, -0.192, 0.597);
\coordinate (X146) at (-2.415, -0.324, -1.707);
\coordinate (X147) at (-3.244, -0.175, -1.685);
\coordinate (X148) at (-0.165, -0.282, -0.697);
\coordinate (X149) at (1.322, 0.002, 0.797);
\coordinate (X150) at (-2.846, -0.333, -2.281);
\coordinate (X151) at (-2.826, -0.158, -1.485);
\coordinate (X152) at (-3.241, -0.329, -0.194);
\coordinate (X153) at (-2.560, -0.216, -0.015);
\coordinate (X154) at (1.534, -0.419, -0.980);
\coordinate (X155) at (0.838, 0.224, -1.447);
\coordinate (X156) at (-2.540, -0.160, -0.045);
\coordinate (X157) at (-0.316, -0.294, -0.132);
\coordinate (X158) at (0.551, -0.415, -1.300);
\coordinate (X159) at (0.284, 0.233, 0.189);
\coordinate (X160) at (-0.816, -0.275, -0.151);
\coordinate (X161) at (-0.800, -0.317, -1.052);
\coordinate (X162) at (-1.694, -0.442, -0.858);
\coordinate (X163) at (-2.720, -0.314, -1.781);
\coordinate (X164) at (1.293, 0.063, 0.946);
\coordinate (X165) at (0.833, -0.008, -1.980);
\coordinate (X166) at (-1.278, -0.297, -1.148);
\coordinate (X167) at (-1.770, 0.090, 0.382);
\coordinate (X168) at (-1.720, 0.590, 0.507);
\coordinate (X169) at (-2.478, -0.288, -1.617);
\coordinate (X170) at (-2.300, -0.293, -1.560);
\coordinate (X171) at (-3.263, 0.170, -0.337);
\coordinate (X172) at (1.948, -0.403, -0.542);
\coordinate (X173) at (-2.294, -0.281, 0.938);
\coordinate (X174) at (1.652, 0.107, 0.439);
\coordinate (X175) at (-2.158, 0.239, -1.419);
\coordinate (X176) at (-2.043, 0.017, -0.016);
\coordinate (X177) at (-2.391, -0.419, 0.606);
\coordinate (X178) at (-2.147, -0.024, -1.601);
\coordinate (X179) at (-1.074, 0.108, -2.125);
\coordinate (X180) at (-1.839, -0.408, -2.112);
\coordinate (X181) at (-2.399, 0.265, 1.130);
\coordinate (X182) at (-0.457, -0.084, -0.489);
\coordinate (X183) at (1.791, -0.299, 1.165);
\coordinate (X184) at (1.657, -0.299, -2.140);
\coordinate (X185) at (-3.018, 0.231, -1.434);
\coordinate (X186) at (-0.004, 0.113, -0.610);
\coordinate (X187) at (-1.375, -0.051, -0.150);
\coordinate (X188) at (-2.111, 0.263, 0.115);
\coordinate (X189) at (-2.435, 0.334, -0.472);
\coordinate (X190) at (-0.718, 0.420, 0.610);
\coordinate (X191) at (-3.153, 0.492, 0.573);
\coordinate (X192) at (0.740, -0.293, -0.890);
\coordinate (X193) at (-2.276, 0.308, -2.150);
\coordinate (X194) at (-1.909, 0.348, -1.880);
\coordinate (X195) at (1.126, -0.423, -0.337);
\coordinate (X196) at (0.730, -0.309, -1.213);
\coordinate (X197) at (0.320, 0.286, 0.624);
\coordinate (X198) at (0.302, 0.055, -1.205);
\coordinate (X199) at (-0.496, -0.099, -0.234);
\coordinate (X200) at (1.793, -0.362, 0.509);
\coordinate (X201) at (-0.874, 0.049, -2.288);
\coordinate (X202) at (1.284, 0.415, 0.433);
\coordinate (X203) at (0.287, 0.486, 0.998);
\coordinate (X204) at (-3.009, 0.042, 0.562);
\coordinate (X205) at (1.547, -0.055, -1.736);
\coordinate (X206) at (1.909, 0.434, -1.790);
\coordinate (X207) at (1.576, 0.487, 0.219);
\coordinate (X208) at (-0.475, -0.103, -2.136);
\coordinate (X209) at (-1.840, 0.354, -2.413);
\coordinate (X210) at (-1.881, -0.231, 0.318);
\coordinate (X211) at (1.466, -0.131, -0.726);
\coordinate (X212) at (0.532, -0.238, -1.294);
\coordinate (X213) at (-1.206, -0.366, -1.400);
\coordinate (X214) at (-1.627, 0.042, 0.618);
\coordinate (X215) at (-3.658, 0.201, -1.629);
\coordinate (X216) at (1.702, -0.298, -0.317);
\coordinate (X217) at (-3.369, 0.281, 0.082);
\coordinate (X218) at (-0.460, -0.550, 1.033);
\coordinate (X219) at (-2.541, 0.405, -1.403);
\coordinate (X220) at (-2.611, -0.388, 0.016);
\coordinate (X221) at (-1.210, 0.018, -0.207);
\coordinate (X222) at (-1.494, 0.115, -1.576);
\coordinate (X223) at (-1.638, -0.266, 0.834);
\coordinate (X224) at (-1.471, -0.485, -1.656);
\coordinate (X225) at (0.377, 0.154, -2.290);
\coordinate (X226) at (-2.410, -0.308, 0.864);
\coordinate (X227) at (-2.857, 0.219, -1.297);
\coordinate (X228) at (-3.188, -0.155, 1.166);
\coordinate (X229) at (1.150, 0.314, -0.503);
\coordinate (X230) at (0.154, -0.322, -1.038);
\coordinate (X231) at (1.415, -0.514, -2.031);
\coordinate (X232) at (-2.716, -0.478, -1.507);
\coordinate (X233) at (0.897, -0.154, -1.088);
\coordinate (X234) at (-1.527, 0.109, -1.117);
\coordinate (X235) at (-0.278, -0.179, 0.332);
\coordinate (X236) at (-1.326, -0.421, -1.075);
\coordinate (X237) at (-0.685, 0.314, -1.047);
\coordinate (X238) at (-0.737, -0.302, -1.085);
\coordinate (X239) at (-3.712, 0.183, -1.792);
\coordinate (X240) at (-0.516, -0.090, 0.296);
\coordinate (X241) at (-0.134, 0.327, -1.456);
\coordinate (X242) at (1.180, 0.109, 0.419);
\coordinate (X243) at (-1.393, -0.070, 0.240);
\coordinate (X244) at (-3.562, -0.299, 1.101);
\coordinate (X245) at (-3.397, 0.119, -1.113);
\coordinate (X246) at (-1.582, -0.208, -0.691);
\coordinate (X247) at (0.304, -0.161, 0.245);
\coordinate (X248) at (0.329, -0.213, -2.176);
\coordinate (X249) at (-2.269, 0.033, -2.109);
\coordinate (X250) at (-1.030, 0.088, -0.690);
\coordinate (X251) at (0.700, -0.365, -2.083);
\coordinate (X252) at (0.442, 0.010, 0.773);
\coordinate (X253) at (0.728, -0.029, -1.044);
\coordinate (X254) at (-0.381, -0.243, -2.004);
\coordinate (X255) at (-1.282, -0.441, 0.223);
\coordinate (X256) at (-2.335, -0.138, -1.457);
\coordinate (X257) at (1.948, 0.477, -2.189);
\coordinate (X258) at (0.164, 0.371, -1.524);
\coordinate (X259) at (-0.646, 0.360, -2.164);
\coordinate (X260) at (1.661, 0.488, -0.149);
\coordinate (X261) at (1.191, 0.327, -0.742);
\coordinate (X262) at (0.914, -0.388, 0.477);
\coordinate (X263) at (-2.495, -0.366, -2.065);
\coordinate (X264) at (0.210, -0.146, 1.133);
\coordinate (X265) at (-3.429, -0.107, 0.290);
\coordinate (X266) at (0.681, -0.099, 0.554);
\coordinate (X267) at (1.350, 0.169, -1.391);
\coordinate (X268) at (-3.665, 0.335, -2.327);
\coordinate (X269) at (0.809, 0.542, -0.696);
\coordinate (X270) at (0.705, -0.043, -0.221);
\coordinate (X271) at (0.437, 0.118, -0.307);
\coordinate (X272) at (0.460, -0.153, -1.673);
\coordinate (X273) at (-1.701, -0.124, -0.938);
\coordinate (X274) at (-2.473, -0.463, -2.348);
\coordinate (X275) at (1.846, -0.154, -0.529);
\coordinate (X276) at (0.742, -0.420, -0.141);
\coordinate (X277) at (1.366, 0.351, -0.107);
\coordinate (X278) at (-2.443, 0.390, 0.824);
\coordinate (X279) at (-0.229, 0.124, -1.325);
\coordinate (X280) at (-2.758, -0.211, -1.511);
\coordinate (X281) at (0.637, -0.015, -2.079);
\coordinate (X282) at (1.896, -0.310, -0.543);
\coordinate (X283) at (0.568, 0.080, -1.714);
\coordinate (X284) at (0.950, -0.209, -1.325);
\coordinate (X285) at (-0.783, 0.028, 0.392);
\coordinate (X286) at (-3.238, 0.443, -1.131);
\coordinate (X287) at (1.132, 0.407, 0.841);
\coordinate (X288) at (-0.618, -0.477, -0.392);
\coordinate (X289) at (-0.854, -0.271, -1.292);
\coordinate (X290) at (-0.988, -0.038, 0.496);
\coordinate (X291) at (0.860, -0.144, 0.970);
\coordinate (X292) at (0.260, 0.171, 0.611);
\coordinate (X293) at (-0.981, -0.477, -0.916);
\coordinate (X294) at (-0.251, 0.513, 0.645);
\coordinate (X295) at (-2.386, 0.133, 0.248);
\coordinate (X296) at (-0.604, 0.437, -0.623);
\coordinate (X297) at (-0.046, 0.423, -1.954);
\coordinate (X298) at (1.453, 0.087, -2.147);
\coordinate (X299) at (-1.974, 0.222, -2.022);
\coordinate (X300) at (-0.609, -0.222, 0.680);
\coordinate (X301) at (1.904, 0.237, -1.743);
\coordinate (X302) at (0.583, -0.272, -2.420);
\coordinate (X303) at (0.088, -0.043, -1.005);
\coordinate (X304) at (2.174, 0.000, -0.262);
\coordinate (X305) at (-2.898, 0.264, 0.837);
\coordinate (X306) at (-2.561, -0.336, 0.811);
\coordinate (X307) at (-1.387, 0.129, -0.454);
\coordinate (X308) at (-2.265, 0.327, -0.256);
\coordinate (X309) at (1.365, -0.219, -1.352);
\coordinate (X310) at (-3.686, 0.145, -0.715);
\coordinate (X311) at (-0.155, -0.291, -2.045);
\coordinate (X312) at (-1.002, -0.320, -1.894);
\coordinate (X313) at (0.137, -0.113, -1.349);
\coordinate (X314) at (-0.895, -0.557, 0.427);
\coordinate (X315) at (-2.177, 0.286, -0.827);
\coordinate (X316) at (-1.157, -0.433, -2.045);
\coordinate (X317) at (-1.633, -0.088, 0.566);
\coordinate (X318) at (0.672, -0.355, -0.085);
\coordinate (X319) at (-2.987, 0.128, 0.601);
\coordinate (X320) at (0.268, -0.015, -2.343);
\coordinate (X321) at (-1.882, -0.082, -1.937);
\coordinate (X322) at (-1.779, -0.434, -1.921);
\coordinate (X323) at (-1.495, -0.234, 0.287);
\coordinate (X324) at (0.181, 0.308, -1.488);
\coordinate (X325) at (-2.776, -0.200, 0.689);
\coordinate (X326) at (-3.644, 0.002, 0.940);
\coordinate (X327) at (-1.787, 0.235, -2.044);
\coordinate (X328) at (-1.181, 0.157, 0.190);
\coordinate (X329) at (0.430, -0.465, -2.080);
\coordinate (X330) at (-2.363, 0.468, -0.853);
\coordinate (X331) at (-2.770, 0.329, 0.919);
\coordinate (X332) at (-0.976, -0.048, 1.148);
\coordinate (X333) at (-0.060, -0.227, 0.852);
\coordinate (X334) at (-3.415, -0.440, -1.123);
\coordinate (X335) at (-1.132, 0.399, 1.188);
\coordinate (X336) at (0.508, -0.026, -0.823);
\coordinate (X337) at (-1.665, 0.517, -2.129);
\coordinate (X338) at (2.414, 0.041, -0.304);
\coordinate (X339) at (2.587, -0.054, -1.050);
\coordinate (X340) at (1.986, 0.464, -1.336);
\coordinate (X341) at (2.217, 0.078, 1.194);
\coordinate (X342) at (1.226, 0.374, -0.154);
\coordinate (X343) at (1.413, 0.371, -0.173);
\coordinate (X344) at (1.941, -0.159, 0.470);
\coordinate (X345) at (1.346, 0.134, -0.880);
\coordinate (X346) at (1.634, -0.250, -2.019);
\coordinate (X347) at (1.305, -0.000, -0.766);
\coordinate (X348) at (2.427, 0.021, -1.318);
\coordinate (X349) at (2.017, 0.227, -1.636);
\coordinate (X350) at (1.411, -0.479, 1.169);
\coordinate (X351) at (1.289, -0.294, -1.099);
\coordinate (X352) at (1.241, -0.291, -0.113);
\coordinate (X353) at (2.541, -0.238, 0.073);
\coordinate (X354) at (2.101, 0.331, -0.222);
\coordinate (X355) at (1.785, 0.131, 0.838);
\coordinate (X356) at (1.222, -0.507, -0.679);
\coordinate (X357) at (2.113, -0.305, 0.899);
\coordinate (X358) at (2.681, -0.309, 0.995);
\coordinate (X359) at (1.788, 0.291, -1.540);
\coordinate (X360) at (2.242, 0.023, 0.662);
\coordinate (X361) at (2.460, 0.020, -2.174);
\coordinate (X362) at (2.619, 0.266, 0.883);
\coordinate (X363) at (1.323, 0.053, -0.418);
\coordinate (X364) at (2.131, -0.436, 0.755);
\coordinate (X365) at (1.628, -0.134, 0.871);
\coordinate (X366) at (1.698, 0.222, -1.743);
\coordinate (X367) at (2.014, -0.276, -0.898);
\coordinate (X368) at (1.671, -0.117, 1.031);
\coordinate (X369) at (1.552, -0.128, -1.286);
\coordinate (X370) at (1.638, -0.296, -1.974);
\coordinate (X371) at (2.094, 0.218, 0.726);
\coordinate (X372) at (1.834, 0.059, -2.137);
\coordinate (X373) at (1.611, -0.211, -0.520);
\coordinate (X374) at (2.076, 0.033, 0.559);
\coordinate (X375) at (2.347, 0.365, 1.104);
\coordinate (X376) at (2.598, -0.474, -1.370);
\coordinate (X377) at (1.404, 0.363, -2.139);
\coordinate (X378) at (2.507, -0.150, -1.797);
\coordinate (X379) at (1.764, -0.208, -1.050);
\coordinate (X380) at (1.502, 0.196, 0.206);
\coordinate (X381) at (1.514, 0.158, 1.091);
\coordinate (X382) at (1.376, 0.008, -1.772);
\coordinate (X383) at (1.323, 0.187, -1.538);
\coordinate (X384) at (1.904, 0.249, -1.986);
\coordinate (X385) at (1.904, 0.252, 0.239);
\coordinate (X386) at (1.264, -0.305, 0.544);
\coordinate (X387) at (1.493, 0.336, -0.250);
\coordinate (X388) at (2.089, -0.312, 0.512);
\coordinate (X389) at (1.699, -0.034, -1.585);
\coordinate (X390) at (2.242, 0.370, -1.326);
\coordinate (X391) at (1.097, -0.460, 0.609);
\coordinate (X392) at (2.125, 0.036, -1.293);
\coordinate (X393) at (1.777, 0.014, -0.063);
\coordinate (X394) at (2.589, -0.342, 1.004);
\coordinate (X395) at (1.738, 0.129, 0.919);
\coordinate (X396) at (2.214, 0.446, -1.798);
\coordinate (X397) at (1.134, 0.163, 0.533);
\coordinate (X398) at (1.526, -0.391, -1.864);
\coordinate (X399) at (2.401, -0.380, -0.974);
\coordinate (X400) at (1.335, -0.115, -2.033);
\coordinate (X401) at (2.123, -0.041, -0.841);
\coordinate (X402) at (1.772, -0.330, 0.295);
\coordinate (X403) at (2.579, -0.355, 1.012);
\coordinate (X404) at (1.290, 0.094, -1.936);
\coordinate (X405) at (1.619, 0.218, -0.786);
\coordinate (X406) at (1.392, -0.097, -1.593);
\coordinate (X407) at (2.745, 0.423, 0.170);
\coordinate (X408) at (2.294, -0.017, 0.584);
\coordinate (X409) at (1.161, 0.234, -1.710);
\coordinate (X410) at (2.351, 0.280, 1.124);
\coordinate (X411) at (1.089, -0.181, -1.151);
\coordinate (X412) at (1.991, -0.191, -0.560);
\coordinate (X413) at (1.884, 0.133, 0.007);
\coordinate (X414) at (1.154, 0.299, -0.616);
\coordinate (X415) at (2.413, -0.229, -2.127);
\coordinate (X416) at (1.681, -0.280, 0.990);
\coordinate (X417) at (1.563, 0.480, 0.822);
\coordinate (X418) at (2.546, 0.119, 0.532);
\coordinate (X419) at (2.291, -0.335, 0.125);
\coordinate (X420) at (1.817, -0.295, -0.598);
\coordinate (X421) at (1.121, -0.616, -1.670);
\coordinate (X422) at (1.704, -0.198, 0.137);
\coordinate (X423) at (1.716, -0.217, 0.743);
\coordinate (X424) at (1.275, 0.119, 0.710);
\coordinate (X425) at (1.223, -0.348, -1.800);
\coordinate (X426) at (1.524, -0.319, 1.005);
\coordinate (X427) at (2.411, 0.169, -0.989);
\coordinate (X428) at (1.946, -0.015, -0.370);
\coordinate (X429) at (1.278, 0.341, -0.270);
\coordinate (X430) at (1.287, -0.034, -0.379);
\coordinate (X431) at (0.967, 0.027, -0.041);
\coordinate (X432) at (1.209, -0.042, -1.269);
\coordinate (X433) at (2.340, 0.429, -0.146);
\coordinate (X434) at (1.335, 0.093, -0.222);
\coordinate (X435) at (2.522, -0.445, 0.006);
\coordinate (X436) at (1.243, -0.110, 1.172);
\coordinate (X437) at (1.701, -0.101, -0.399);
\coordinate (X438) at (2.611, 0.244, -0.802);
\coordinate (X439) at (2.165, 0.003, -1.069);
\coordinate (X440) at (1.781, 0.106, 0.776);
\coordinate (X441) at (2.485, 0.074, 0.441);
\coordinate (X442) at (1.067, 0.045, -1.749);
\coordinate (X443) at (2.247, 0.162, 0.975);
\coordinate (X444) at (1.192, -0.359, 1.160);
\coordinate (X445) at (1.072, -0.447, -2.514);
\coordinate (X446) at (2.701, 0.353, -0.713);
\coordinate (X447) at (2.199, -0.416, -1.506);
\coordinate (X448) at (1.436, -0.456, -1.994);
\coordinate (X449) at (1.964, -0.128, -1.319);
\coordinate (X450) at (2.163, 0.049, -2.209);
\coordinate (X451) at (2.451, 0.288, -0.988);
\coordinate (X452) at (2.683, 0.100, 0.407);
\coordinate (X453) at (2.135, 0.245, 0.822);
\coordinate (X454) at (1.450, -0.169, -0.267);
\coordinate (X455) at (1.430, -0.408, -1.372);
\coordinate (X456) at (2.649, 0.080, -1.022);
\coordinate (X457) at (2.416, 0.231, -1.533);
\coordinate (X458) at (1.012, -0.368, -1.667);
\coordinate (X459) at (2.223, 0.418, -1.395);
\coordinate (X460) at (1.852, 0.274, 1.155);
\coordinate (X461) at (1.810, 0.065, -0.030);
\coordinate (X462) at (1.555, 0.127, 0.818);
\coordinate (X463) at (1.226, 0.180, -2.425);
\coordinate (X464) at (1.322, -0.007, 1.159);
\coordinate (X465) at (2.001, -0.396, -0.572);
\coordinate (X466) at (2.288, -0.027, -2.361);
\coordinate (X467) at (1.269, 0.578, -0.565);
\coordinate (X468) at (1.525, -0.379, -0.910);
\coordinate (X469) at (2.525, 0.489, -0.616);
\coordinate (X470) at (1.852, -0.021, -0.366);
\coordinate (X471) at (2.120, -0.329, 0.616);
\coordinate (X472) at (1.527, 0.358, -1.898);
\coordinate (X473) at (2.023, -0.036, 0.751);
\coordinate (X474) at (1.093, 0.130, 0.192);
\coordinate (X475) at (1.917, 0.237, 0.828);
\coordinate (X476) at (1.683, -0.411, -2.083);
\coordinate (X477) at (1.563, 0.277, 1.037);
\coordinate (X478) at (2.406, 0.016, -0.296);
\coordinate (X479) at (1.231, -0.111, -0.182);
\coordinate (X480) at (1.107, -0.249, 0.531);
\coordinate (X481) at (1.958, -0.037, 0.662);
\coordinate (X482) at (2.342, -0.356, -0.471);
\coordinate (X483) at (2.415, -0.188, 0.480);
\coordinate (X484) at (1.896, -0.305, -0.705);
\coordinate (X485) at (1.608, -0.467, -2.295);
\coordinate (X486) at (2.466, -0.204, 0.158);
\coordinate (X487) at (1.436, 0.336, -1.118);
\coordinate (X488) at (1.331, 0.187, -0.031);
\coordinate (X489) at (1.805, -0.290, -2.047);
\coordinate (X490) at (2.252, -0.085, -0.238);
\coordinate (X491) at (2.207, 0.271, -1.559);
\coordinate (X492) at (2.262, 0.443, -2.000);
\coordinate (X493) at (1.091, -0.057, -1.240);
\coordinate (X494) at (1.426, 0.287, -1.354);
\coordinate (X495) at (1.483, 0.273, -0.229);
\coordinate (X496) at (2.304, -0.182, -0.045);
\coordinate (X497) at (1.220, 0.014, -0.263);
\coordinate (X498) at (1.673, 0.408, -2.436);
\coordinate (X499) at (2.096, 0.654, 0.307);
\coordinate (X500) at (2.662, -0.314, -0.342);
\coordinate (X501) at (1.377, 0.174, -1.511);
\coordinate (X502) at (1.948, -0.046, -1.868);
\coordinate (X503) at (1.137, -0.260, -1.163);
\coordinate (X504) at (2.448, 0.170, 0.129);
\coordinate (X505) at (1.188, 0.280, 1.166);
\coordinate (X506) at (1.130, 0.183, 0.106);
\coordinate (X507) at (1.245, -0.116, -0.083);
\coordinate (X508) at (1.977, 0.029, -0.431);
\coordinate (X509) at (2.312, -0.015, -2.141);
\coordinate (X510) at (1.826, 0.325, -0.197);
\coordinate (X511) at (1.135, 0.218, -1.504);
\coordinate (X512) at (1.309, -0.471, -0.822);
\coordinate (X513) at (2.257, -0.014, -1.298);
\coordinate (X514) at (2.254, -0.490, -2.088);
\coordinate (X515) at (1.739, 0.422, 0.246);
\coordinate (X516) at (1.776, -0.275, 0.718);
\coordinate (X517) at (2.652, -0.446, 0.246);
\coordinate (X518) at (1.536, 0.186, 0.300);
\coordinate (X519) at (2.193, 0.246, -0.528);
\coordinate (X520) at (2.382, 0.019, -1.630);
\coordinate (X521) at (2.228, 0.194, -0.959);
\coordinate (X522) at (2.480, 0.477, -1.154);
\coordinate (X523) at (2.739, -0.331, -1.323);
\coordinate (X524) at (1.308, 0.210, 0.766);
\coordinate (X525) at (1.336, -0.109, 0.561);
\coordinate (X526) at (1.789, 0.499, -0.369);
\coordinate (X527) at (2.753, 0.204, 0.665);
\coordinate (X528) at (1.218, 0.438, -0.451);
\coordinate (X529) at (1.323, -0.536, 0.412);
\coordinate (X530) at (1.010, 0.174, -1.423);
\coordinate (X531) at (2.462, 0.405, 0.259);
\coordinate (X532) at (2.130, -0.224, -0.098);
\coordinate (X533) at (2.221, 0.094, -0.619);
\coordinate (X534) at (1.925, 0.215, -0.670);
\coordinate (X535) at (1.173, -0.349, -1.655);
\coordinate (X536) at (1.980, 0.021, -0.668);
\coordinate (X537) at (2.110, -0.285, 0.873);
\coordinate (X538) at (1.594, 0.160, -1.891);
\coordinate (X539) at (1.239, 0.508, -1.278);
\coordinate (X540) at (2.314, -0.101, 0.731);
\coordinate (X541) at (2.234, 0.113, -0.880);
\coordinate (X542) at (1.319, -0.366, -0.911);
\coordinate (X543) at (2.248, 0.410, 0.873);
\coordinate (X544) at (1.459, 0.440, 0.784);
\coordinate (X545) at (2.065, -0.218, -0.193);
\coordinate (X546) at (1.894, 0.323, 0.201);
\coordinate (X547) at (1.647, 0.503, -1.870);
\coordinate (X548) at (1.754, -0.406, 1.117);
\coordinate (X549) at (1.538, 0.349, -1.947);
\coordinate (X550) at (2.271, -0.008, -1.914);
\coordinate (X551) at (1.443, -0.442, -0.038);
\coordinate (X552) at (1.545, 0.045, -0.786);
\coordinate (X553) at (1.523, 0.236, -2.073);
\coordinate (X554) at (2.543, 0.381, 1.022);
\coordinate (X555) at (1.983, 0.368, -1.473);
\coordinate (X556) at (2.482, -0.031, -2.171);
\coordinate (X557) at (2.409, 0.170, -1.943);
\coordinate (X558) at (1.220, 0.466, 0.917);
\coordinate (X559) at (2.489, 0.537, 0.353);
\coordinate (X560) at (1.883, -0.084, -0.848);
\coordinate (X561) at (1.846, 0.179, 0.462);
\coordinate (X562) at (2.607, 0.032, 0.523);
\coordinate (X563) at (2.129, 0.126, 1.118);
\coordinate (X564) at (1.409, 0.099, -1.682);
\coordinate (X565) at (1.694, 0.004, 0.819);
\coordinate (X566) at (1.837, 0.082, -1.954);
\coordinate (X567) at (1.494, -0.156, -0.057);
\coordinate (X568) at (0.971, -0.321, -1.009);
\coordinate (X569) at (2.764, -0.205, -0.145);
\coordinate (X570) at (1.269, 0.023, -0.926);
\coordinate (X571) at (1.464, 0.052, -2.260);
\coordinate (X572) at (1.026, -0.265, -2.222);
\coordinate (X573) at (1.964, 0.079, -0.954);
\coordinate (X574) at (2.562, -0.149, -1.950);
\coordinate (X575) at (2.096, -0.442, -0.706);
\coordinate (X576) at (1.875, 0.321, -0.040);
\coordinate (X577) at (2.203, 0.406, -1.716);
\coordinate (X578) at (1.401, -0.012, -0.174);
\coordinate (X579) at (1.634, 0.444, 1.012);
\coordinate (X580) at (2.550, 0.307, -2.441);
\coordinate (X581) at (2.135, -0.480, -1.094);
\coordinate (X582) at (1.078, 0.105, 0.943);
\coordinate (X583) at (1.141, -0.084, -0.067);
\coordinate (X584) at (1.569, -0.268, -0.249);
\coordinate (X585) at (2.210, -0.505, -1.966);
\coordinate (X586) at (1.561, 0.573, 0.848);
\coordinate (X587) at (2.089, -0.203, 0.563);
\coordinate (X588) at (2.001, 0.369, 1.111);
\coordinate (X589) at (1.256, 0.443, -2.070);
\coordinate (X590) at (1.908, -0.359, -2.425);
\coordinate (X591) at (1.733, -0.048, -0.098);
\coordinate (X592) at (1.920, -0.490, -1.730);
\coordinate (X593) at (1.977, -0.150, 1.071);
\coordinate (X594) at (2.109, 0.233, 0.971);
\coordinate (X595) at (1.791, 0.089, -1.159);
\coordinate (X596) at (1.633, 0.247, -0.142);
\coordinate (X597) at (2.484, -0.044, -0.866);
\coordinate (X598) at (1.889, -0.087, 0.501);
\coordinate (X599) at (2.181, 0.107, -0.456);
\coordinate (X600) at (1.348, 0.016, -1.710);
\coordinate (X601) at (2.378, 0.005, -1.635);
\coordinate (X602) at (0.992, 0.183, 0.777);
\coordinate (X603) at (1.575, -0.307, -0.323);
\coordinate (X604) at (1.450, 0.135, 0.612);
\coordinate (X605) at (1.734, 0.173, -1.723);
\coordinate (X606) at (1.782, -0.522, 0.225);
\coordinate (X607) at (2.763, -0.183, -2.072);
\coordinate (X608) at (1.026, -0.086, -1.608);
\coordinate (X609) at (0.995, 0.331, -0.157);
\coordinate (X610) at (1.456, 0.304, -1.880);
\coordinate (X611) at (1.487, 0.451, -0.363);
\coordinate (X612) at (1.690, -0.165, 0.130);
\coordinate (X613) at (1.291, 0.124, 0.189);
\coordinate (X614) at (2.308, 0.308, -0.267);
\coordinate (X615) at (1.333, -0.235, -1.367);
\coordinate (X616) at (1.055, -0.135, -1.128);
\coordinate (X617) at (2.658, 0.053, -0.770);
\coordinate (X618) at (2.078, -0.268, -0.280);
\coordinate (X619) at (2.094, 0.041, -0.393);
\coordinate (X620) at (2.556, 0.452, 0.587);
\coordinate (X621) at (1.937, 0.320, -1.383);
\coordinate (X622) at (1.641, -0.590, 0.016);
\coordinate (X623) at (2.638, 0.283, 0.183);
\coordinate (X624) at (1.219, 0.366, -0.976);
\coordinate (X625) at (2.517, 0.414, -1.604);
\coordinate (X626) at (1.776, 0.398, -0.076);
\coordinate (X627) at (2.465, 0.164, -0.580);
\coordinate (X628) at (1.668, 0.090, 0.070);
\coordinate (X629) at (1.952, 0.558, -1.372);
\coordinate (X630) at (1.219, 0.268, -0.211);
\coordinate (X631) at (2.363, 0.309, -2.099);
\coordinate (X632) at (2.450, -0.053, -0.020);
\coordinate (X633) at (2.128, 0.505, -2.423);
\coordinate (X634) at (1.877, 0.135, 1.168);
\coordinate (X635) at (2.165, -0.337, -0.946);
\coordinate (X636) at (1.695, 0.216, -0.988);
\coordinate (X637) at (1.438, 0.505, -2.164);
\coordinate (X638) at (1.589, -0.456, 1.151);
\coordinate (X639) at (2.503, 0.209, -1.789);
\coordinate (X640) at (2.236, 0.317, 0.898);
\coordinate (X641) at (2.302, 0.441, 0.482);
\coordinate (X642) at (1.120, -0.020, -2.009);
\coordinate (X643) at (1.696, -0.027, -2.089);
\coordinate (X644) at (2.528, 0.384, -3.005);
\coordinate (X645) at (0.953, -0.150, -3.160);
\coordinate (X646) at (-2.992, -0.105, -2.853);
\coordinate (X647) at (1.997, -0.300, -2.218);
\coordinate (X648) at (-0.288, -0.053, -2.858);
\coordinate (X649) at (-2.235, 0.167, -2.828);
\coordinate (X650) at (-3.134, -0.358, -2.720);
\coordinate (X651) at (2.620, -0.248, -2.424);
\coordinate (X652) at (0.769, 0.492, -2.168);
\coordinate (X653) at (-0.157, 0.138, -2.153);
\coordinate (X654) at (-1.276, -0.196, -3.639);
\coordinate (X655) at (2.035, 0.256, -3.295);
\coordinate (X656) at (-0.005, -0.123, -3.534);
\coordinate (X657) at (3.254, -0.303, -3.568);
\coordinate (X658) at (0.277, 0.291, -3.526);
\coordinate (X659) at (0.798, 0.092, -3.464);
\coordinate (X660) at (-3.239, 0.137, -3.050);
\coordinate (X661) at (2.933, 0.259, -1.877);
\coordinate (X662) at (-2.526, 0.458, -2.747);
\coordinate (X663) at (-1.822, -0.534, -3.565);
\coordinate (X664) at (1.035, -0.009, -3.206);
\coordinate (X665) at (0.307, -0.190, -2.666);
\coordinate (X666) at (-1.659, 0.272, -2.260);
\coordinate (X667) at (-0.788, -0.158, -2.971);
\coordinate (X668) at (1.884, -0.419, -3.284);
\coordinate (X669) at (-3.891, 0.089, -2.844);
\coordinate (X670) at (2.159, -0.148, -3.031);
\coordinate (X671) at (1.917, 0.267, -2.967);
\coordinate (X672) at (-0.945, -0.230, -1.810);
\coordinate (X673) at (-3.531, 0.510, -2.390);
\coordinate (X674) at (-0.427, -0.409, -2.699);
\coordinate (X675) at (-1.357, -0.244, -2.421);
\coordinate (X676) at (3.315, 0.043, -2.453);
\coordinate (X677) at (-4.017, 0.037, -3.514);
\coordinate (X678) at (0.185, 0.442, -2.495);
\coordinate (X679) at (-3.924, -0.059, -2.690);
\coordinate (X680) at (-1.467, 0.482, -2.277);
\coordinate (X681) at (0.250, -0.029, -3.176);
\coordinate (X682) at (-3.699, -0.092, -2.804);
\coordinate (X683) at (0.811, 0.275, -3.614);
\coordinate (X684) at (-1.340, -0.354, -3.215);
\coordinate (X685) at (2.049, -0.477, -2.824);
\coordinate (X686) at (-3.134, 0.425, -2.714);
\coordinate (X687) at (-2.732, 0.015, -2.348);
\coordinate (X688) at (3.132, -0.402, -2.061);
\coordinate (X689) at (2.868, 0.353, -2.561);
\coordinate (X690) at (0.454, -0.341, -2.361);
\coordinate (X691) at (-0.377, 0.222, -2.914);
\coordinate (X692) at (1.262, 0.437, -3.260);
\coordinate (X693) at (2.149, 0.016, -2.115);
\coordinate (X694) at (-1.125, -0.118, -2.006);
\coordinate (X695) at (-2.583, 0.452, -2.774);
\coordinate (X696) at (-0.405, -0.067, -2.538);
\coordinate (X697) at (-2.053, -0.399, -3.058);
\coordinate (X698) at (-4.420, 0.393, -1.998);
\coordinate (X699) at (-1.323, 0.178, -3.017);
\coordinate (X700) at (0.911, 0.304, -2.035);
\coordinate (X701) at (-1.418, 0.310, -3.226);
\coordinate (X702) at (3.316, -0.420, -2.467);
\coordinate (X703) at (0.754, 0.142, -3.290);
\coordinate (X704) at (2.901, -0.384, -2.541);
\coordinate (X705) at (-2.662, -0.161, -2.656);
\coordinate (X706) at (-1.102, -0.418, -3.383);
\coordinate (X707) at (-1.329, 0.288, -2.053);
\coordinate (X708) at (-3.755, -0.073, -3.439);
\coordinate (X709) at (-4.403, 0.177, -2.684);
\coordinate (X710) at (-3.044, -0.206, -3.523);
\coordinate (X711) at (2.144, 0.521, -3.360);
\coordinate (X712) at (-2.741, 0.411, -1.989);
\coordinate (X713) at (-1.259, -0.318, -3.491);
\coordinate (X714) at (0.078, 0.010, -3.529);
\coordinate (X715) at (0.122, -0.399, -2.304);
\coordinate (X716) at (-2.096, -0.421, -2.656);
\coordinate (X717) at (-1.208, 0.367, -2.755);
\coordinate (X718) at (-2.253, 0.266, -3.195);
\coordinate (X719) at (2.694, -0.002, -2.654);
\coordinate (X720) at (-3.946, -0.183, -2.125);
\coordinate (X721) at (1.951, -0.188, -3.212);
\coordinate (X722) at (1.938, 0.459, -3.359);
\coordinate (X723) at (-0.915, -0.069, -2.184);
\coordinate (X724) at (-3.888, -0.333, -2.338);
\coordinate (X725) at (-4.054, 0.013, -2.645);
\coordinate (X726) at (-1.864, -0.084, -2.677);
\coordinate (X727) at (-3.299, 0.078, -2.139);
\coordinate (X728) at (1.513, -0.378, -3.394);
\coordinate (X729) at (-2.437, -0.116, -2.804);
\coordinate (X730) at (0.769, -0.437, -3.510);
\coordinate (X731) at (-1.554, 0.142, -3.301);
\coordinate (X732) at (0.505, -0.205, -2.096);
\coordinate (X733) at (2.542, -0.152, -3.066);
\coordinate (X734) at (-1.149, -0.376, -2.403);
\coordinate (X735) at (2.016, 0.191, -2.218);
\coordinate (X736) at (-1.372, -0.307, -2.376);
\coordinate (X737) at (-1.736, 0.145, -3.105);
\coordinate (X738) at (-3.846, 0.549, -3.351);
\coordinate (X739) at (3.339, 0.542, -2.156);
\coordinate (X740) at (0.700, 0.072, -2.105);
\coordinate (X741) at (-2.318, -0.032, -2.481);
\coordinate (X742) at (-1.221, -0.077, -3.006);
\coordinate (X743) at (-0.111, 0.401, -3.244);
\coordinate (X744) at (2.870, 0.169, -2.195);
\coordinate (X745) at (-0.148, 0.330, -3.580);
\coordinate (X746) at (2.083, -0.324, -2.143);
\coordinate (X747) at (3.352, -0.233, -3.247);
\coordinate (X748) at (1.691, -0.247, -2.093);
\coordinate (X749) at (-3.679, -0.420, -1.990);
\coordinate (X750) at (0.732, 0.283, -3.238);
\coordinate (X751) at (0.880, 0.252, -2.551);
\coordinate (X752) at (0.786, 0.039, -2.888);
\coordinate (X753) at (-2.416, 0.334, -3.138);
\coordinate (X754) at (0.883, -0.192, -2.414);
\coordinate (X755) at (1.539, -0.051, -3.542);
\coordinate (X756) at (-3.290, 0.089, -2.189);
\coordinate (X757) at (-4.154, 0.196, -2.974);
\coordinate (X758) at (-0.828, 0.409, -2.926);
\coordinate (X759) at (-0.842, -0.445, -3.407);
\coordinate (X760) at (-2.396, -0.562, -2.472);
\coordinate (X761) at (-1.166, 0.071, -3.207);
\coordinate (X762) at (-2.270, 0.097, -2.091);
\coordinate (X763) at (-4.174, 0.485, -2.615);
\coordinate (X764) at (-0.151, -0.022, -3.569);
\coordinate (X765) at (-3.902, 0.138, -3.088);
\coordinate (X766) at (2.834, -0.082, -3.331);
\coordinate (X767) at (1.124, -0.130, -2.636);
\coordinate (X768) at (1.034, 0.439, -2.258);
\coordinate (X769) at (0.878, 0.161, -1.984);
\coordinate (X770) at (-2.204, -0.501, -3.170);
\coordinate (X771) at (-2.770, 0.263, -2.426);
\coordinate (X772) at (0.090, -0.360, -2.373);
\coordinate (X773) at (-1.921, 0.106, -2.630);
\coordinate (X774) at (-1.789, -0.446, -3.375);
\coordinate (X775) at (2.169, 0.403, -2.385);
\coordinate (X776) at (-3.727, -0.020, -2.510);
\coordinate (X777) at (1.836, -0.247, -3.599);
\coordinate (X778) at (0.981, -0.105, -3.254);
\coordinate (X779) at (-4.401, 0.081, -2.212);
\coordinate (X780) at (3.155, 0.134, -2.641);
\coordinate (X781) at (-3.859, -0.042, -2.867);
\coordinate (X782) at (0.270, -0.195, -3.076);
\coordinate (X783) at (-3.629, -0.168, -3.260);
\coordinate (X784) at (-3.123, 0.455, -2.875);
\coordinate (X785) at (-0.191, 0.316, -1.847);
\coordinate (X786) at (0.055, 0.281, -2.953);
\coordinate (X787) at (-2.133, -0.110, -2.363);
\coordinate (X788) at (1.001, -0.119, -3.401);
\coordinate (X789) at (0.453, -0.339, -2.580);
\coordinate (X790) at (0.903, 0.258, -2.302);
\coordinate (X791) at (2.277, -0.054, -2.384);
\coordinate (X792) at (0.380, -0.153, -3.518);
\coordinate (X793) at (-2.335, -0.026, -2.564);
\coordinate (X794) at (2.242, -0.238, -3.279);
\coordinate (X795) at (3.119, -0.246, -2.706);
\coordinate (X796) at (0.067, 0.212, -3.410);
\coordinate (X797) at (-4.142, -0.248, -2.441);
\coordinate (X798) at (-0.212, -0.280, -2.516);
\coordinate (X799) at (2.033, -0.336, -2.698);
\coordinate (X800) at (0.949, -0.118, -3.082);
\coordinate (X801) at (0.415, 0.375, -2.182);
\coordinate (X802) at (0.090, 0.231, -2.991);
\coordinate (X803) at (0.655, -0.073, -3.312);
\coordinate (X804) at (1.194, 0.138, -3.146);
\coordinate (X805) at (2.666, -0.580, -3.115);
\coordinate (X806) at (-4.310, 0.260, -2.477);
\coordinate (X807) at (-1.898, 0.065, -2.905);
\coordinate (X808) at (1.444, 0.077, -2.782);
\coordinate (X809) at (2.949, -0.251, -3.232);
\coordinate (X810) at (-0.003, 0.363, -2.948);
\coordinate (X811) at (-3.879, -0.157, -2.739);
\coordinate (X812) at (-3.353, 0.233, -1.828);
\coordinate (X813) at (-0.889, -0.173, -2.954);
\coordinate (X814) at (-3.714, 0.388, -2.957);
\coordinate (X815) at (-1.543, 0.136, -2.869);
\coordinate (X816) at (0.577, -0.376, -2.201);
\coordinate (X817) at (2.917, 0.169, -2.041);
\coordinate (X818) at (-3.324, 0.002, -2.673);
\coordinate (X819) at (0.159, -0.146, -3.002);
\coordinate (X820) at (-3.443, -0.025, -3.302);
\coordinate (X821) at (1.274, -0.199, -3.431);
\coordinate (X822) at (-0.191, 0.047, -2.258);
\coordinate (X823) at (0.061, -0.142, -2.143);
\coordinate (X824) at (-0.216, -0.296, -2.675);
\coordinate (X825) at (2.762, -0.125, -3.023);
\coordinate (X826) at (-3.501, -0.306, -2.992);
\coordinate (X827) at (0.179, -0.359, -2.032);
\coordinate (X828) at (1.389, 0.157, -2.189);
\coordinate (X829) at (-3.933, -0.006, -2.326);
\coordinate (X830) at (2.133, 0.370, -3.080);
\coordinate (X831) at (2.953, -0.522, -2.152);
\coordinate (X832) at (3.145, -0.434, -2.445);
\coordinate (X833) at (-4.358, -0.081, -2.649);
\coordinate (X834) at (0.159, 0.463, -2.515);
\coordinate (X835) at (-0.850, 0.184, -2.068);
\coordinate (X836) at (-4.424, 0.466, -3.506);
\coordinate (X837) at (1.960, -0.216, -3.355);
\coordinate (X838) at (-0.958, 0.066, -2.906);
\coordinate (X839) at (-4.103, 0.085, -1.993);
\coordinate (X840) at (-1.427, -0.329, -2.846);
\coordinate (X841) at (-4.131, 0.302, -2.143);
\coordinate (X842) at (0.157, 0.004, -2.341);
\coordinate (X843) at (-0.136, 0.261, -2.470);
\coordinate (X844) at (1.581, 0.133, -2.926);
\coordinate (X845) at (3.024, -0.052, -2.592);
\coordinate (X846) at (-2.705, 0.132, -2.570);
\coordinate (X847) at (-2.946, -0.392, -2.600);
\coordinate (X848) at (1.567, -0.004, -3.233);
\coordinate (X849) at (0.651, -0.325, -2.862);
\coordinate (X850) at (-3.224, -0.366, -3.206);
\coordinate (X851) at (-1.517, -0.430, -2.844);
\coordinate (X852) at (-0.412, -0.005, -3.061);
\coordinate (X853) at (2.349, -0.203, -2.674);
\coordinate (X854) at (-4.097, -0.408, -2.650);
\coordinate (X855) at (0.054, 0.396, -2.695);
\coordinate (X856) at (3.057, -0.341, -3.298);
\coordinate (X857) at (-4.075, -0.236, -2.684);
\coordinate (X858) at (0.360, -0.403, -1.984);
\coordinate (X859) at (2.167, -0.179, -3.544);
\coordinate (X860) at (-3.145, -0.301, -3.321);
\coordinate (X861) at (-0.346, -0.188, -3.004);
\coordinate (X862) at (3.322, 0.197, -1.971);
\coordinate (X863) at (-3.330, -0.054, -2.493);
\coordinate (X864) at (-3.766, -0.459, -2.725);
\coordinate (X865) at (0.654, -0.112, -2.811);
\coordinate (X866) at (-1.263, -0.478, -2.969);
\coordinate (X867) at (-3.241, -0.452, -1.941);
\coordinate (X868) at (0.272, 0.279, -3.104);
\coordinate (X869) at (-1.482, -0.277, -3.398);
\coordinate (X870) at (-3.005, 0.151, -2.452);
\coordinate (X871) at (-0.286, -0.131, -1.954);
\coordinate (X872) at (-3.918, -0.166, -2.922);
\coordinate (X873) at (1.647, 0.456, -3.015);
\coordinate (X874) at (2.394, 0.384, -3.199);
\coordinate (X875) at (-1.496, -0.222, -1.971);
\coordinate (X876) at (-3.022, 0.358, -2.949);
\coordinate (X877) at (1.201, 0.052, -2.673);
\coordinate (X878) at (2.096, 0.305, -2.131);
\coordinate (X879) at (-3.965, 0.147, -3.440);
\coordinate (X880) at (-1.230, 0.031, -2.656);
\coordinate (X881) at (-0.357, 0.461, -3.427);
\coordinate (X882) at (0.696, -0.161, -3.346);
\coordinate (X883) at (-3.171, 0.527, -2.079);
\coordinate (X884) at (2.649, 0.506, -3.265);
\coordinate (X885) at (-1.587, 0.162, -2.769);
\coordinate (X886) at (-1.371, -0.138, -2.517);
\coordinate (X887) at (-0.039, -0.367, -2.726);
\coordinate (X888) at (-0.244, 0.157, -3.263);
\coordinate (X889) at (1.335, -0.526, -2.953);
\coordinate (X890) at (1.842, 0.131, -3.201);
\coordinate (X891) at (1.069, 0.055, -2.137);
\coordinate (X892) at (1.364, -0.094, -2.828);
\coordinate (X893) at (-3.409, -0.206, -2.946);
\coordinate (X894) at (0.181, -0.112, -3.099);
\coordinate (X895) at (-4.324, 0.067, -2.939);
\coordinate (X896) at (1.366, -0.371, -2.450);
\coordinate (X897) at (2.973, -0.314, -2.709);
\coordinate (X898) at (-3.704, 0.099, -2.703);
\coordinate (X899) at (-1.288, 0.093, -2.010);
\coordinate (X900) at (-3.078, -0.309, -2.172);
\coordinate (X901) at (0.031, 0.324, -2.377);
\coordinate (X902) at (1.920, -0.116, -2.252);
\coordinate (X903) at (2.775, 0.069, -3.213);
\coordinate (X904) at (-2.459, -0.313, -3.308);
\coordinate (X905) at (-2.196, 0.196, -2.469);
\coordinate (X906) at (-1.141, 0.244, -3.452);
\coordinate (X907) at (-3.855, -0.299, -2.714);
\coordinate (X908) at (-2.850, -0.113, -2.893);
\coordinate (X909) at (1.967, -0.381, -2.456);
\coordinate (X910) at (0.710, 0.203, -1.995);
\coordinate (X911) at (-4.388, -0.314, -2.086);
\coordinate (X912) at (-0.705, -0.021, -2.605);
\coordinate (X913) at (0.885, 0.401, -1.875);
\coordinate (X914) at (1.229, -0.099, -2.204);
\coordinate (X915) at (-4.184, -0.215, -2.010);
\coordinate (X916) at (-2.341, -0.187, -3.350);
\coordinate (X917) at (2.227, -0.028, -2.484);
\coordinate (X918) at (-2.588, 0.280, -2.393);
\coordinate (X919) at (-2.083, -0.010, -3.200);
\coordinate (X920) at (3.266, 0.181, -1.886);
\coordinate (X921) at (-2.107, 0.256, -2.354);
\coordinate (X922) at (0.979, 0.285, -2.928);
\coordinate (X923) at (-3.511, 0.080, -2.416);
\coordinate (X924) at (0.093, -0.253, -2.721);
\coordinate (X925) at (-2.032, -0.050, -2.401);
\coordinate (X926) at (1.395, -0.350, -2.777);
\coordinate (X927) at (-2.370, -0.320, -2.348);
\coordinate (X928) at (2.718, -0.121, -2.198);
\coordinate (X929) at (2.567, 0.286, -3.206);
\coordinate (X930) at (3.130, -0.094, -2.958);
\coordinate (X931) at (-4.042, 0.016, -3.310);
\coordinate (X932) at (-2.515, -0.176, -2.117);
\coordinate (X933) at (2.251, -0.029, -2.254);
\coordinate (X934) at (2.231, 0.265, -3.342);
\coordinate (X935) at (1.023, 0.365, -2.409);
\coordinate (X936) at (-1.942, 0.035, -2.495);
\coordinate (X937) at (-0.471, -0.393, -3.089);
\coordinate (X938) at (1.861, 0.429, -3.390);
\coordinate (X939) at (2.970, -0.108, -2.464);
\coordinate (X940) at (1.499, 0.248, -2.113);
\coordinate (X941) at (-2.087, 0.303, -3.362);
\coordinate (X942) at (1.021, 0.299, -2.457);
\coordinate (X943) at (-2.519, 0.383, -3.280);
\coordinate (X944) at (-4.111, 0.259, -2.834);
\coordinate (X945) at (2.313, -0.117, -3.389);
\coordinate (X946) at (2.125, -0.002, -3.211);
\coordinate (X947) at (1.349, -0.033, -2.536);
\coordinate (X948) at (-1.000, 0.362, -2.244);
\coordinate (X949) at (1.057, -0.447, -2.112);
\coordinate (X950) at (0.869, 0.204, -3.029);
\coordinate (X951) at (2.566, 0.176, -3.545);
\coordinate (X952) at (-1.262, 0.305, -3.427);
\coordinate (X953) at (3.077, 0.229, -2.413);
\coordinate (X954) at (-2.473, -0.270, -1.996);
\coordinate (X955) at (-2.054, 0.231, -2.959);
\coordinate (X956) at (-3.394, -0.500, -2.650);
\coordinate (X957) at (3.106, 0.047, -3.074);
\coordinate (X958) at (-1.824, 0.030, -2.697);
\coordinate (X959) at (2.361, 0.161, -2.668);
\coordinate (X960) at (-3.406, 0.407, -3.116);
\coordinate (X961) at (-4.005, 0.261, -2.645);
\coordinate (X962) at (-1.245, -0.102, -2.326);
\coordinate (X963) at (-2.927, 0.360, -2.398);
\coordinate (X964) at (-1.335, 0.049, -2.965);
\coordinate (X965) at (1.409, 0.162, -3.057);
\coordinate (X966) at (0.102, 0.468, -2.769);
\coordinate (X967) at (2.720, -0.180, -3.443);
\coordinate (X968) at (-2.912, -0.023, -3.191);
\coordinate (X969) at (-4.499, 0.381, -2.139);
\coordinate (X970) at (1.296, -0.214, -3.421);
\coordinate (X971) at (-3.916, 0.212, -1.998);
\coordinate (X972) at (-1.150, -0.427, -2.841);
\coordinate (X973) at (-1.840, -0.131, -2.516);
\coordinate (X974) at (1.249, -0.394, -3.582);
\coordinate (X975) at (3.262, -0.210, -3.388);
\coordinate (X976) at (-2.935, -0.380, -2.872);
\coordinate (X977) at (1.963, -0.116, -2.783);
\coordinate (X978) at (0.810, -0.077, -2.176);
\coordinate (X979) at (2.346, -0.455, -2.128);
\coordinate (X980) at (-0.868, 0.569, -2.795);
\coordinate (X981) at (3.284, 0.162, -3.213);
\coordinate (X982) at (-0.219, 0.487, -2.065);
\coordinate (X983) at (-3.748, 0.186, -2.841);
\coordinate (X984) at (-4.487, 0.004, -3.212);
\coordinate (X985) at (2.023, -0.077, -2.168);
\coordinate (X986) at (-4.701, -0.171, -3.083);
\coordinate (X987) at (-2.641, -0.371, -3.387);
\coordinate (X988) at (-0.173, -0.158, -2.845);
\coordinate (X989) at (-1.453, 0.364, -2.023);
\coordinate (X990) at (-0.617, -0.222, -3.561);
\coordinate (X991) at (3.072, -0.398, -3.121);
\coordinate (X992) at (-2.284, -0.115, -3.321);
\coordinate (X993) at (1.728, -0.216, -2.663);

\def\numPoints{994}
\def\numCameras{3}


==> fig/tasks/bunny_registration.tex <==
% Source point cloud
\coordinate (s0) at (-0.0498,-0.2524,0.1652);
\coordinate (s1) at (0.3278,-0.2210,0.1240);
\coordinate (s2) at (0.1848,0.1356,-0.1318);
\coordinate (s3) at (0.2077,-0.3166,-0.1020);
\coordinate (s4) at (0.0158,0.4005,-0.1523);
\coordinate (s5) at (-0.2201,0.3294,0.0979);
\coordinate (s6) at (0.4626,-0.1568,0.0567);
\coordinate (s7) at (-0.0078,-0.1844,-0.1881);
\coordinate (s8) at (0.3302,0.0641,-0.1000);
\coordinate (s9) at (-0.1103,0.2731,-0.0417);
\coordinate (s10) at (0.2659,0.0968,-0.1230);
\coordinate (s11) at (-0.1905,0.3080,-0.1063);
\coordinate (s12) at (-0.1885,0.2122,-0.0918);
\coordinate (s13) at (-0.3078,0.0959,0.1054);
\coordinate (s14) at (-0.1099,0.0909,0.1493);
\coordinate (s15) at (0.0736,-0.2955,-0.0136);
\coordinate (s16) at (0.1603,-0.3143,0.1573);
\coordinate (s17) at (-0.1699,0.2339,0.1288);
\coordinate (s18) at (-0.3221,0.3156,0.0403);
\coordinate (s19) at (-0.3102,0.2823,-0.0188);
\coordinate (s20) at (0.2785,-0.2265,-0.1662);
\coordinate (s21) at (0.2852,-0.2593,-0.1025);
\coordinate (s22) at (-0.2067,-0.1550,0.0967);
\coordinate (s23) at (0.3062,-0.2335,-0.1091);
\coordinate (s24) at (-0.0299,-0.0642,-0.2097);
\coordinate (s25) at (0.3492,-0.1919,0.1164);
\coordinate (s26) at (-0.1455,-0.2488,0.0822);
\coordinate (s27) at (-0.1724,-0.2828,0.0478);
\coordinate (s28) at (0.0578,0.4898,-0.1609);
\coordinate (s29) at (0.1083,-0.1376,-0.2425);
\coordinate (s30) at (0.4386,-0.1965,0.0894);
\coordinate (s31) at (-0.0168,0.4366,-0.1377);
\coordinate (s32) at (-0.2046,-0.3087,0.1607);
\coordinate (s33) at (-0.3358,0.1982,-0.0244);
\coordinate (s34) at (-0.0190,-0.2376,-0.1667);
\coordinate (s35) at (-0.1556,-0.2044,-0.0608);
\coordinate (s36) at (0.2619,-0.1064,0.2126);
\coordinate (s37) at (0.0189,-0.1287,0.2021);
\coordinate (s38) at (0.0365,0.4717,-0.1715);
\coordinate (s39) at (-0.0369,-0.3151,0.1732);
\coordinate (s40) at (0.0418,-0.3129,0.2211);
\coordinate (s41) at (0.4070,-0.2252,0.1031);
\coordinate (s42) at (-0.1401,-0.2509,0.0717);
\coordinate (s43) at (-0.1968,0.2911,-0.1685);
\coordinate (s44) at (-0.1501,-0.2400,0.1281);
\coordinate (s45) at (-0.2058,0.1124,-0.1100);
\coordinate (s46) at (-0.3552,0.1298,0.0271);
\coordinate (s47) at (0.2511,0.1123,0.1426);
\coordinate (s48) at (-0.1887,-0.1700,0.0779);
\coordinate (s49) at (-0.2995,0.1908,-0.0730);
\coordinate (s50) at (-0.1616,-0.1663,-0.0821);
\coordinate (s51) at (0.0174,0.4826,-0.1150);
\coordinate (s52) at (0.0168,0.4117,-0.1168);
\coordinate (s53) at (-0.1349,-0.2406,0.0695);
\coordinate (s54) at (-0.2470,0.0885,0.1800);
\coordinate (s55) at (0.2519,-0.2398,-0.1722);
\coordinate (s56) at (0.3896,-0.2718,0.0584);
\coordinate (s57) at (-0.1609,0.0765,0.1580);
\coordinate (s58) at (0.2453,-0.2294,0.1866);
\coordinate (s59) at (-0.1528,-0.3214,-0.0556);
\coordinate (s60) at (-0.2924,0.2629,-0.0517);
\coordinate (s61) at (-0.2027,-0.1317,-0.1079);
\coordinate (s62) at (-0.1872,-0.2589,0.1565);
\coordinate (s63) at (0.1878,0.1968,-0.0344);
\coordinate (s64) at (-0.3345,0.2475,0.1176);
\coordinate (s65) at (-0.2631,0.3029,0.1488);
\coordinate (s66) at (0.3078,-0.1605,0.1688);
\coordinate (s67) at (0.2153,-0.1598,0.2272);
\coordinate (s68) at (0.0865,-0.2919,-0.1912);
\coordinate (s69) at (0.4680,-0.1728,0.0292);
\coordinate (s70) at (-0.1391,-0.3197,0.0760);
\coordinate (s71) at (-0.3091,0.0224,-0.0616);
\coordinate (s72) at (0.3761,0.0304,0.0088);
\coordinate (s73) at (0.3624,-0.1587,0.1057);
\coordinate (s74) at (-0.1194,-0.0883,-0.1505);
\coordinate (s75) at (-0.2087,-0.2965,0.0287);
\coordinate (s76) at (0.1195,0.1862,0.0940);
\coordinate (s77) at (0.1701,0.1746,0.1136);
\coordinate (s78) at (-0.0172,-0.2768,0.2232);
\coordinate (s79) at (0.4566,-0.1857,0.0674);
\coordinate (s80) at (0.0092,-0.1865,-0.2147);
\coordinate (s81) at (-0.2284,0.0477,-0.1274);
\coordinate (s82) at (0.1766,0.1818,-0.0757);
\coordinate (s83) at (-0.3067,0.0706,-0.0404);
\coordinate (s84) at (0.0917,0.1948,0.0084);
\coordinate (s85) at (0.4383,-0.2390,0.0484);
\coordinate (s86) at (-0.0613,-0.1638,0.1700);
\coordinate (s87) at (0.0554,-0.1352,0.2384);
\coordinate (s88) at (0.2096,-0.0452,0.2359);
\coordinate (s89) at (-0.0828,0.0864,0.1518);
\coordinate (s90) at (0.0015,-0.2125,0.1524);
\coordinate (s91) at (-0.1151,-0.3154,0.1688);
\coordinate (s92) at (-0.1996,0.3327,0.0771);
\coordinate (s93) at (0.1699,-0.0429,0.2532);
\coordinate (s94) at (0.1462,0.0963,0.1752);
\coordinate (s95) at (0.1415,-0.2934,0.0791);
\coordinate (s96) at (-0.0377,-0.0737,-0.1872);
\coordinate (s97) at (-0.3107,0.3176,0.0135);
\coordinate (s98) at (-0.2219,0.2939,-0.2372);
\coordinate (s99) at (-0.2408,0.3151,0.1328);
\coordinate (s100) at (-0.2585,0.3441,-0.0913);
\coordinate (s101) at (0.0529,-0.0571,0.2560);
\coordinate (s102) at (-0.2851,0.2544,-0.0667);
\coordinate (s103) at (0.3664,0.0213,0.0836);
\coordinate (s104) at (-0.3294,0.1250,0.1945);
\coordinate (s105) at (0.1423,-0.2575,-0.1963);
\coordinate (s106) at (-0.0267,-0.1779,-0.1374);
\coordinate (s107) at (0.1748,-0.1711,0.2461);
\coordinate (s108) at (-0.1068,0.0138,0.1818);
\coordinate (s109) at (0.0502,-0.0364,-0.2574);
\coordinate (s110) at (-0.1821,0.1639,0.1752);
\coordinate (s111) at (0.2378,0.0921,0.1563);
\coordinate (s112) at (0.3116,-0.2912,-0.0611);
\coordinate (s113) at (0.1167,-0.3063,-0.1846);
\coordinate (s114) at (-0.3195,-0.0587,0.0280);
\coordinate (s115) at (-0.1578,-0.1796,-0.0687);
\coordinate (s116) at (-0.0138,-0.3035,-0.2120);
\coordinate (s117) at (0.1567,-0.0669,0.2530);
\coordinate (s118) at (0.1539,0.0891,0.1757);
\coordinate (s119) at (-0.1832,-0.3115,0.1835);
\coordinate (s120) at (-0.2645,-0.1374,0.0118);
\coordinate (s121) at (-0.1589,-0.1647,-0.0848);
\coordinate (s122) at (0.4432,-0.2369,0.0205);
\coordinate (s123) at (-0.0953,0.3522,-0.0152);
\coordinate (s124) at (0.0726,0.1869,0.0587);
\coordinate (s125) at (0.0708,-0.1529,0.2365);
\coordinate (s126) at (-0.1925,0.3990,-0.2980);
\coordinate (s127) at (0.3198,0.1230,0.0345);
\coordinate (s128) at (-0.2554,0.3401,-0.1845);
\coordinate (s129) at (-0.2601,-0.0402,0.1562);
\coordinate (s130) at (0.0800,-0.2098,0.2244);
\coordinate (s131) at (-0.0184,-0.1061,0.1644);
\coordinate (s132) at (-0.1083,-0.1690,-0.1183);
\coordinate (s133) at (0.0300,0.0305,-0.1806);
\coordinate (s134) at (0.2211,-0.1138,0.2335);
\coordinate (s135) at (0.1707,-0.2945,-0.1105);
\coordinate (s136) at (-0.3530,0.1938,0.0753);
\coordinate (s137) at (-0.1174,-0.0936,-0.1478);
\coordinate (s138) at (-0.1000,-0.3180,0.1031);
\coordinate (s139) at (-0.1544,-0.1280,0.1538);
\coordinate (s140) at (-0.2806,0.3291,0.0559);
\coordinate (s141) at (-0.2384,0.1382,-0.0962);
\coordinate (s142) at (-0.0525,0.1171,-0.1342);
\coordinate (s143) at (-0.0243,-0.1391,-0.1791);
\coordinate (s144) at (-0.2403,0.1943,0.2223);
\coordinate (s145) at (0.2574,-0.0019,-0.1746);
\coordinate (s146) at (0.3457,0.0884,0.0282);
\coordinate (s147) at (0.3603,0.0269,-0.0759);
\coordinate (s148) at (-0.3063,0.3138,-0.0080);
\coordinate (s149) at (0.3149,-0.1539,0.1650);
\coordinate (s150) at (-0.1610,0.2991,-0.0596);
\coordinate (s151) at (-0.2136,0.3250,-0.3231);
\coordinate (s152) at (-0.2620,-0.1142,-0.0803);
\coordinate (s153) at (-0.1762,-0.1818,-0.0352);
\coordinate (s154) at (-0.1853,0.1095,-0.1232);
\coordinate (s155) at (0.0715,-0.1646,-0.2478);
\coordinate (s156) at (0.2800,-0.0279,0.1999);
\coordinate (s157) at (-0.0182,-0.3074,-0.2130);
\coordinate (s158) at (-0.1454,-0.1568,0.1261);
\coordinate (s159) at (-0.3111,0.0451,-0.0484);
\coordinate (s160) at (-0.3530,0.1702,0.0989);
\coordinate (s161) at (0.1701,-0.0833,-0.2348);
\coordinate (s162) at (-0.0488,0.3500,-0.0369);
\coordinate (s163) at (0.1808,0.1999,0.0514);
\coordinate (s164) at (0.2653,0.0654,0.1608);
\coordinate (s165) at (-0.0814,-0.2304,-0.1098);
\coordinate (s166) at (-0.1625,0.2351,0.1235);
\coordinate (s167) at (0.0978,-0.2948,0.0682);
\coordinate (s168) at (0.0228,-0.0201,-0.2444);
\coordinate (s169) at (-0.1351,-0.0068,0.1841);
\coordinate (s170) at (-0.1358,-0.1026,0.1738);
\coordinate (s171) at (-0.1806,-0.1787,-0.0476);
\coordinate (s172) at (0.3740,-0.1623,0.0999);
\coordinate (s173) at (-0.3299,0.1975,-0.0341);
\coordinate (s174) at (0.0843,-0.0073,-0.2427);
\coordinate (s175) at (0.0777,-0.0689,-0.2580);
\coordinate (s176) at (-0.2422,-0.2950,-0.0199);
\coordinate (s177) at (-0.0942,-0.0476,0.1809);
\coordinate (s178) at (-0.1623,0.1127,-0.1304);
\coordinate (s179) at (-0.0019,0.1636,-0.0521);
\coordinate (s180) at (0.3518,-0.1655,-0.0985);
\coordinate (s181) at (-0.3366,0.1077,0.1657);
\coordinate (s182) at (0.2518,-0.0992,-0.1971);
\coordinate (s183) at (-0.1261,-0.2175,-0.0958);
\coordinate (s184) at (-0.0514,0.3426,-0.1125);
\coordinate (s185) at (-0.2344,0.3486,-0.2893);
\coordinate (s186) at (0.1759,-0.2906,0.1145);
\coordinate (s187) at (-0.2745,0.0457,-0.0981);
\coordinate (s188) at (0.1381,-0.3064,0.0348);
\coordinate (s189) at (0.0369,-0.0556,-0.2589);
\coordinate (s190) at (-0.1272,-0.3164,0.1155);
\coordinate (s191) at (0.2894,-0.2898,0.1053);
\coordinate (s192) at (-0.0599,-0.0524,0.1826);
\coordinate (s193) at (-0.0957,-0.2472,-0.1076);
\coordinate (s194) at (0.0436,0.3515,-0.1092);
\coordinate (s195) at (-0.1850,0.3400,-0.1857);
\coordinate (s196) at (-0.3362,0.2130,0.1314);
\coordinate (s197) at (0.2961,0.1350,-0.0547);
\coordinate (s198) at (-0.0018,0.4405,-0.0952);
\coordinate (s199) at (0.4108,-0.1079,0.0224);
\coordinate (s200) at (-0.2137,0.0067,0.1748);
\coordinate (s201) at (-0.2676,0.3900,-0.1929);
\coordinate (s202) at (0.3007,-0.0658,0.1844);
\coordinate (s203) at (0.0668,0.1194,0.1537);
\coordinate (s204) at (-0.3565,0.1300,0.0541);
\coordinate (s205) at (-0.1259,-0.2974,0.1958);
\coordinate (s206) at (0.3105,-0.2493,0.1215);
\coordinate (s207) at (-0.1283,0.2784,0.0213);
\coordinate (s208) at (-0.2619,-0.0522,0.1509);
\coordinate (s209) at (0.2675,-0.3127,-0.0479);
\coordinate (s210) at (-0.0137,-0.3142,0.1901);
\coordinate (s211) at (-0.2325,-0.0339,0.1727);
\coordinate (s212) at (0.0602,0.4348,-0.1514);
\coordinate (s213) at (-0.3265,0.0455,0.0562);
\coordinate (s214) at (-0.0754,0.3030,-0.0287);
\coordinate (s215) at (0.0004,-0.1974,-0.1970);
\coordinate (s216) at (0.2525,0.0930,-0.1327);
\coordinate (s217) at (-0.2270,0.0370,0.1646);
\coordinate (s218) at (-0.0345,0.3168,-0.0555);
\coordinate (s219) at (-0.3479,0.1804,0.1144);
\coordinate (s220) at (0.3779,0.0264,0.0028);
\coordinate (s221) at (0.0552,-0.2026,0.2197);
\coordinate (s222) at (0.0275,-0.1193,0.2219);
\coordinate (s223) at (-0.1439,-0.3204,0.0680);
\coordinate (s224) at (0.4071,-0.1573,0.1039);
\coordinate (s225) at (-0.0847,0.0079,0.1752);
\coordinate (s226) at (-0.2432,-0.2998,-0.0173);
\coordinate (s227) at (0.3721,-0.0011,0.0860);
\coordinate (s228) at (-0.0770,0.4058,-0.0426);
\coordinate (s229) at (0.2902,-0.0641,0.1936);
\coordinate (s230) at (0.3817,-0.2797,0.0417);
\coordinate (s231) at (-0.1806,0.3288,0.0834);
\coordinate (s232) at (-0.1139,-0.1269,0.1613);
\coordinate (s233) at (0.0949,0.1943,-0.0077);
\coordinate (s234) at (-0.1746,-0.0332,-0.1599);
\coordinate (s235) at (0.0323,0.1672,-0.0611);
\coordinate (s236) at (-0.1187,0.2967,-0.0704);
\coordinate (s237) at (0.0578,0.1864,0.0348);
\coordinate (s238) at (-0.0060,-0.1101,-0.2371);
\coordinate (s239) at (0.1848,0.1091,0.1614);
\coordinate (s240) at (-0.2300,0.0693,0.1491);
\coordinate (s241) at (-0.0637,0.0994,-0.1463);
\coordinate (s242) at (0.0116,-0.2431,0.2145);
\coordinate (s243) at (0.2549,0.1450,0.1198);
\coordinate (s244) at (-0.1101,-0.3198,-0.1298);
\coordinate (s245) at (-0.3353,-0.0136,0.0300);
\coordinate (s246) at (0.2628,-0.2134,-0.1876);
\coordinate (s247) at (0.0607,0.0112,0.2294);
\coordinate (s248) at (-0.2633,0.3322,0.0237);
\coordinate (s249) at (-0.0457,0.4413,-0.0807);
\coordinate (s250) at (-0.3084,0.0962,0.1088);
\coordinate (s251) at (0.2096,-0.3122,-0.0318);
\coordinate (s252) at (-0.1905,0.2952,-0.1317);
\coordinate (s253) at (0.4657,-0.1892,0.0218);
\coordinate (s254) at (0.3204,0.0546,0.1327);
\coordinate (s255) at (-0.2677,0.3247,0.0974);
\coordinate (s256) at (-0.2751,0.0958,-0.0686);
\coordinate (s257) at (-0.2219,-0.1705,0.0460);
\coordinate (s258) at (-0.2287,0.0073,-0.1377);
\coordinate (s259) at (-0.1985,0.3251,0.1085);
\coordinate (s260) at (-0.0850,0.1132,0.1300);
\coordinate (s261) at (-0.2405,-0.0027,0.1705);
\coordinate (s262) at (0.4565,-0.1830,-0.0311);
\coordinate (s263) at (0.3800,0.0140,0.0237);
\coordinate (s264) at (0.0921,0.1948,0.0081);
\coordinate (s265) at (-0.0897,-0.2221,0.1570);
\coordinate (s266) at (0.0906,0.1582,-0.1027);
\coordinate (s267) at (0.0020,-0.0006,-0.1998);
\coordinate (s268) at (-0.0517,0.3237,-0.0978);
\coordinate (s269) at (0.1022,-0.2941,-0.0285);
\coordinate (s270) at (-0.2256,0.3344,-0.0557);
\coordinate (s271) at (-0.0140,0.1419,0.0967);
\coordinate (s272) at (0.1761,-0.2753,-0.1798);
\coordinate (s273) at (0.4608,-0.2007,0.0350);
\coordinate (s274) at (-0.1605,0.1088,0.1403);
\coordinate (s275) at (0.2294,0.0622,0.1820);
\coordinate (s276) at (-0.1520,-0.0823,0.1824);
\coordinate (s277) at (-0.2825,0.2945,0.1522);
\coordinate (s278) at (0.2334,-0.1295,-0.2104);
\coordinate (s279) at (-0.3596,0.1576,0.0775);
\coordinate (s280) at (-0.3315,0.0052,0.0652);
\coordinate (s281) at (0.1803,0.2025,0.0110);
\coordinate (s282) at (-0.2382,0.3568,-0.2773);
\coordinate (s283) at (0.3131,0.0799,0.1244);
\coordinate (s284) at (-0.2131,0.0554,-0.1325);
\coordinate (s285) at (-0.2276,0.4360,-0.2933);
\coordinate (s286) at (0.2557,0.1176,-0.1181);
\coordinate (s287) at (0.3836,-0.0059,0.0331);
\coordinate (s288) at (0.0329,0.1491,0.1110);
\coordinate (s289) at (-0.0220,0.3957,-0.1398);
\coordinate (s290) at (-0.3287,0.0401,-0.0029);
\coordinate (s291) at (0.2017,0.0211,-0.1781);
\coordinate (s292) at (0.1499,0.2020,-0.0022);
\coordinate (s293) at (-0.2164,-0.1102,0.1485);
\coordinate (s294) at (-0.1641,-0.2575,0.0906);
\coordinate (s295) at (0.4507,-0.2054,-0.0265);
\coordinate (s296) at (-0.0182,-0.3014,-0.2126);
\coordinate (s297) at (-0.2512,-0.1085,-0.0960);
\coordinate (s298) at (-0.0180,0.1583,0.0661);
\coordinate (s299) at (0.2822,0.1447,-0.0562);
\coordinate (s300) at (-0.0363,0.3195,-0.0882);
\coordinate (s301) at (-0.1614,-0.2426,0.1439);
\coordinate (s302) at (0.3486,-0.2611,0.1099);
\coordinate (s303) at (0.1676,0.1920,-0.0553);
\coordinate (s304) at (0.2641,0.1091,0.1374);
\coordinate (s305) at (0.3770,-0.2820,-0.0210);
\coordinate (s306) at (-0.2318,0.3372,-0.3055);
\coordinate (s307) at (0.0399,0.1811,-0.0106);
\coordinate (s308) at (0.0247,0.3547,-0.0681);
\coordinate (s309) at (0.0390,0.3942,-0.1542);
\coordinate (s310) at (-0.2026,0.0550,-0.1398);
\coordinate (s311) at (-0.1097,-0.1866,0.1448);
\coordinate (s312) at (-0.1564,-0.0927,-0.1529);
\coordinate (s313) at (-0.1953,0.3271,-0.1092);
\coordinate (s314) at (-0.2031,-0.0953,0.1640);
\coordinate (s315) at (0.0977,-0.2719,-0.1902);
\coordinate (s316) at (-0.3475,0.1776,0.1334);
\coordinate (s317) at (0.3461,-0.0768,-0.1205);
\coordinate (s318) at (-0.3166,0.0972,0.1212);
\coordinate (s319) at (0.1905,-0.1163,0.2463);
\coordinate (s320) at (0.2306,-0.0418,0.2221);
\coordinate (s321) at (-0.0215,-0.1774,-0.1529);
\coordinate (s322) at (0.2360,-0.3137,0.1352);
\coordinate (s323) at (-0.1896,-0.1861,0.0146);
\coordinate (s324) at (0.0002,0.1522,0.0805);
\coordinate (s325) at (0.0990,-0.0124,-0.2433);
\coordinate (s326) at (0.1304,0.1541,-0.1082);
\coordinate (s327) at (-0.2666,-0.1171,-0.0655);
\coordinate (s328) at (-0.1896,0.0905,-0.1314);
\coordinate (s329) at (-0.3270,0.0993,0.1320);
\coordinate (s330) at (-0.1101,0.1392,-0.1238);
\coordinate (s331) at (0.0504,0.0008,-0.2335);
\coordinate (s332) at (-0.3114,0.1742,-0.0677);
\coordinate (s333) at (0.2698,-0.0307,0.2064);
\coordinate (s334) at (-0.0401,-0.3179,0.0548);
\coordinate (s335) at (-0.3322,0.1090,0.1122);
\coordinate (s336) at (0.2596,0.1723,-0.0120);
\coordinate (s337) at (-0.2609,0.3249,0.1027);
\coordinate (s338) at (0.2962,0.1137,-0.0876);
\coordinate (s339) at (-0.0175,0.0945,-0.1468);
\coordinate (s340) at (-0.1523,0.0786,-0.1487);
\coordinate (s341) at (-0.3202,0.2794,0.1323);
\coordinate (s342) at (-0.2093,0.3333,0.0236);
\coordinate (s343) at (-0.3202,0.2551,-0.0053);
\coordinate (s344) at (-0.2095,0.2928,-0.2141);
\coordinate (s345) at (-0.2847,0.0075,-0.1000);
\coordinate (s346) at (0.3760,-0.0891,0.0908);
\coordinate (s347) at (-0.3331,0.2497,0.1358);
\coordinate (s348) at (0.2919,0.0237,-0.1496);
\coordinate (s349) at (-0.1426,0.2556,0.0932);
\coordinate (s350) at (-0.3204,0.1842,0.2026);
\coordinate (s351) at (-0.3509,0.1684,0.1513);
\coordinate (s352) at (0.1808,-0.0017,-0.2171);
\coordinate (s353) at (0.1305,-0.2968,0.2022);
\coordinate (s354) at (0.3080,-0.1107,-0.1604);
\coordinate (s355) at (0.3680,0.0509,-0.0018);
\coordinate (s356) at (0.4014,-0.1538,0.1019);
\coordinate (s357) at (-0.1263,0.2952,0.0181);
\coordinate (s358) at (-0.2604,0.1581,0.2320);
\coordinate (s359) at (-0.0098,0.0136,0.1879);
\coordinate (s360) at (0.0753,-0.2425,0.2069);
\coordinate (s361) at (-0.0002,-0.2470,-0.1904);
\coordinate (s362) at (0.2285,0.1714,0.0975);
\coordinate (s363) at (-0.0083,-0.2217,-0.1751);
\coordinate (s364) at (0.1890,0.1927,0.0783);
\coordinate (s365) at (0.1732,-0.3105,0.0761);
\coordinate (s366) at (-0.1497,0.0116,0.1819);
\coordinate (s367) at (-0.0794,0.1115,0.1316);
\coordinate (s368) at (0.0871,-0.0342,0.2527);
\coordinate (s369) at (0.0965,-0.0719,0.2586);
\coordinate (s370) at (0.1748,-0.1525,-0.2259);
\coordinate (s371) at (0.3407,0.0602,-0.0833);
\coordinate (s372) at (0.0697,-0.2089,-0.2301);
\coordinate (s373) at (0.0849,0.3852,-0.1604);
\coordinate (s374) at (0.2027,0.0940,-0.1525);
\coordinate (s375) at (-0.1350,0.2470,-0.0486);
\coordinate (s376) at (0.0250,0.1551,-0.0873);
\coordinate (s377) at (-0.2974,0.0877,0.1439);
\coordinate (s378) at (0.0904,0.1890,-0.0382);
\coordinate (s379) at (-0.0323,-0.3170,0.0803);
\coordinate (s380) at (-0.0925,-0.0266,0.1789);
\coordinate (s381) at (0.3293,0.1073,0.0649);
\coordinate (s382) at (0.3351,-0.2939,0.0671);
\coordinate (s383) at (0.1648,-0.2898,-0.1808);
\coordinate (s384) at (0.1064,-0.0291,-0.2468);
\coordinate (s385) at (0.4073,-0.1134,0.0499);
\coordinate (s386) at (0.0714,-0.2291,-0.2202);
\coordinate (s387) at (0.1632,-0.3178,0.0333);
\coordinate (s388) at (-0.1587,0.1726,0.1590);
\coordinate (s389) at (-0.2343,0.2541,-0.0949);
\coordinate (s390) at (0.0453,0.1430,0.1269);
\coordinate (s391) at (0.0930,0.3954,-0.1590);
\coordinate (s392) at (-0.1704,-0.1805,0.0654);
\coordinate (s393) at (-0.1691,-0.2399,-0.0303);
\coordinate (s394) at (-0.3261,0.2129,-0.0364);
\coordinate (s395) at (-0.0478,0.3360,-0.0316);
\coordinate (s396) at (0.2836,-0.2864,0.1188);
\coordinate (s397) at (-0.2773,-0.0114,-0.1077);
\coordinate (s398) at (-0.2901,-0.0336,-0.0895);
\coordinate (s399) at (0.1531,-0.2260,-0.2133);
\coordinate (s400) at (-0.0289,0.0722,-0.1578);
\coordinate (s401) at (-0.1004,-0.3212,-0.0340);
\coordinate (s402) at (-0.1374,0.3077,0.0409);
\coordinate (s403) at (-0.2531,0.3622,-0.2305);
\coordinate (s404) at (-0.2115,0.2610,-0.1074);
\coordinate (s405) at (-0.2047,-0.3214,-0.0593);
\coordinate (s406) at (0.2982,0.1410,0.0705);
\coordinate (s407) at (-0.0835,-0.1784,-0.1180);
\coordinate (s408) at (0.0648,0.4884,-0.1908);
\coordinate (s409) at (0.0252,-0.2937,-0.1249);
\coordinate (s410) at (0.1120,-0.2484,0.2070);
\coordinate (s411) at (-0.0729,0.1769,-0.0712);
\coordinate (s412) at (0.0646,-0.2948,-0.0412);
\coordinate (s413) at (-0.2450,-0.0726,0.1546);
\coordinate (s414) at (0.2518,0.0074,0.2018);
\coordinate (s415) at (0.0274,0.1445,0.1149);
\coordinate (s416) at (-0.2115,0.2547,0.1774);
\coordinate (s417) at (0.0110,-0.1250,0.1895);
\coordinate (s418) at (0.0455,-0.2963,0.0142);
\coordinate (s419) at (0.2475,0.0818,0.1595);
\coordinate (s420) at (0.1219,0.0136,0.2367);
\coordinate (s421) at (-0.3011,0.2449,0.1903);
\coordinate (s422) at (-0.2330,-0.0733,0.1616);
\coordinate (s423) at (0.0279,-0.2944,0.1138);
\coordinate (s424) at (-0.0162,0.3726,-0.1334);
\coordinate (s425) at (-0.2533,0.4213,-0.3089);
\coordinate (s426) at (0.0669,0.0811,-0.1612);
\coordinate (s427) at (-0.1875,0.3755,-0.3577);
\coordinate (s428) at (-0.0502,-0.3202,-0.1634);
\coordinate (s429) at (-0.1544,0.1701,0.1562);
\coordinate (s430) at (-0.2917,0.0757,-0.0647);
\coordinate (s431) at (-0.2195,0.2482,0.1880);
\coordinate (s432) at (0.2444,-0.3142,-0.0655);
\coordinate (s433) at (0.3659,0.0313,-0.0600);
\coordinate (s434) at (0.3813,-0.1289,-0.0448);
\coordinate (s435) at (-0.0593,-0.3128,0.0831);
\coordinate (s436) at (0.3417,0.0359,-0.1030);
\coordinate (s437) at (0.3723,-0.2791,-0.0392);
\coordinate (s438) at (0.2929,-0.2892,0.1027);
\coordinate (s439) at (-0.1265,0.2859,0.0179);
\coordinate (s440) at (-0.0797,-0.3108,0.1765);
\coordinate (s441) at (-0.2605,0.2916,-0.1187);
\coordinate (s442) at (0.0061,-0.1022,0.1959);
\coordinate (s443) at (-0.2211,-0.0468,-0.1461);
\coordinate (s444) at (0.2162,0.1890,0.0657);
\coordinate (s445) at (0.0157,0.1755,0.0198);
\coordinate (s446) at (-0.1381,-0.1726,0.1055);
\coordinate (s447) at (0.0596,-0.2444,0.2068);
\coordinate (s448) at (-0.0192,-0.2834,0.2248);
\coordinate (s449) at (-0.2843,0.3165,-0.0291);
\coordinate (s450) at (-0.1118,0.2257,0.0257);
\coordinate (s451) at (-0.2887,0.3158,-0.0255);
\coordinate (s452) at (0.1554,0.1070,0.1691);
\coordinate (s453) at (0.0256,0.3762,-0.1393);
\coordinate (s454) at (-0.0342,-0.1161,-0.1711);
\coordinate (s455) at (0.0631,-0.1706,0.2331);
\coordinate (s456) at (0.1682,0.1946,-0.0485);
\coordinate (s457) at (0.2861,-0.0542,-0.1745);
\coordinate (s458) at (-0.1896,0.3772,-0.2986);
\coordinate (s459) at (-0.3075,0.2541,0.1769);
\coordinate (s460) at (0.2356,-0.0484,0.2220);
\coordinate (s461) at (-0.1776,0.3243,-0.0415);
\coordinate (s462) at (0.2663,0.1697,0.0052);
\coordinate (s463) at (0.1511,0.0494,-0.1704);
\coordinate (s464) at (-0.1811,-0.2527,0.1545);
\coordinate (s465) at (0.1949,0.0533,0.1910);
\coordinate (s466) at (0.1485,-0.2211,-0.2135);
\coordinate (s467) at (-0.0390,-0.0641,-0.1820);
\coordinate (s468) at (0.1425,0.1965,-0.0403);
\coordinate (s469) at (-0.0493,0.0659,0.1558);
\coordinate (s470) at (-0.3094,-0.0350,-0.0657);
\coordinate (s471) at (-0.0508,0.3623,-0.0525);
\coordinate (s472) at (-0.3328,0.2601,0.0185);
\coordinate (s473) at (0.3991,-0.2009,-0.0810);
\coordinate (s474) at (-0.1355,0.2447,-0.0496);
\coordinate (s475) at (0.0582,-0.2486,-0.2083);
\coordinate (s476) at (-0.3187,0.0813,0.0419);
\coordinate (s477) at (-0.2032,-0.3215,-0.0640);
\coordinate (s478) at (-0.1452,-0.2586,0.0341);
\coordinate (s479) at (-0.1835,-0.0438,-0.1557);
\coordinate (s480) at (0.2266,-0.3152,0.0729);
\coordinate (s481) at (-0.3070,0.0740,-0.0362);
\coordinate (s482) at (0.3250,0.0007,0.1602);
\coordinate (s483) at (-0.2753,0.0767,0.1292);
\coordinate (s484) at (-0.1840,0.3297,0.0821);
\coordinate (s485) at (-0.1917,-0.1704,0.0751);
\coordinate (s486) at (-0.0773,0.4123,-0.0998);
\coordinate (s487) at (0.3460,-0.2970,0.0361);
\coordinate (s488) at (-0.0939,0.1623,0.0759);
\coordinate (s489) at (0.2059,0.0320,0.2055);
\coordinate (s490) at (-0.2109,0.0062,0.1755);
\coordinate (s491) at (0.3922,-0.0917,0.0203);
\coordinate (s492) at (0.0127,-0.1121,-0.2501);
\coordinate (s493) at (0.0284,-0.1016,0.2316);
\coordinate (s494) at (-0.0212,0.4365,-0.1341);
\coordinate (s495) at (0.2906,-0.2520,-0.1136);
\coordinate (s496) at (0.2051,0.1795,0.1002);
\coordinate (s497) at (-0.0482,0.0879,-0.1533);
\coordinate (s498) at (0.3167,-0.3052,0.0461);
\coordinate (s499) at (0.0737,0.1915,0.0285);
\coordinate (s500) at (0.3664,-0.2883,0.0353);
\coordinate (s501) at (0.2470,0.0317,0.1967);
\coordinate (s502) at (-0.1588,0.1619,-0.0910);
\coordinate (s503) at (-0.0927,0.1938,0.0249);
\coordinate (s504) at (-0.3601,0.1538,0.0381);
\coordinate (s505) at (0.2468,-0.2448,0.1724);
\coordinate (s506) at (0.2539,-0.1006,-0.1964);
\coordinate (s507) at (0.0841,-0.1411,0.2410);
\coordinate (s508) at (-0.0685,-0.0482,0.1808);
\coordinate (s509) at (0.1576,-0.0886,0.2506);
\coordinate (s510) at (0.1911,0.1039,-0.1519);
\coordinate (s511) at (-0.2132,0.2252,0.1851);
\coordinate (s512) at (0.0605,-0.2415,-0.2131);
\coordinate (s513) at (-0.0932,0.3544,-0.0172);
\coordinate (s514) at (0.1519,0.2024,0.0026);
\coordinate (s515) at (-0.1679,0.3277,-0.0475);
\coordinate (s516) at (0.0535,0.4991,-0.1631);
\coordinate (s517) at (-0.2575,-0.1048,0.1215);
\coordinate (s518) at (0.0669,-0.1731,-0.2449);
\coordinate (s519) at (-0.0902,0.1543,0.0844);
\coordinate (s520) at (-0.2711,0.0396,0.1361);
\coordinate (s521) at (0.2923,-0.0960,0.1883);
\coordinate (s522) at (-0.1758,-0.2456,-0.0174);
\coordinate (s523) at (-0.3040,-0.0709,0.0705);
\coordinate (s524) at (0.2026,-0.3153,0.1487);
\coordinate (s525) at (-0.1999,0.1965,0.1779);
\coordinate (s526) at (-0.2603,0.1308,0.2293);
\coordinate (s527) at (-0.2622,0.3676,-0.1372);
\coordinate (s528) at (0.2006,-0.3059,0.1102);
\coordinate (s529) at (0.1720,-0.2395,-0.2041);
\coordinate (s530) at (-0.2271,-0.1589,-0.0449);
\coordinate (s531) at (0.1763,0.1638,-0.1004);
\coordinate (s532) at (-0.2219,0.3376,-0.3349);
\coordinate (s533) at (-0.1039,-0.1702,-0.1195);
\coordinate (s534) at (0.3796,0.0033,-0.0436);
\coordinate (s535) at (0.1477,0.0994,0.1741);
\coordinate (s536) at (-0.1835,0.2504,0.1398);
\coordinate (s537) at (0.3055,-0.1984,0.1611);
\coordinate (s538) at (0.0844,0.1741,-0.0783);
\coordinate (s539) at (-0.0623,0.3537,-0.1158);
\coordinate (s540) at (0.2679,0.0046,0.1989);
\coordinate (s541) at (-0.3062,0.2591,0.1734);
\coordinate (s542) at (-0.3181,-0.0677,0.0283);
\coordinate (s543) at (0.3621,-0.1131,-0.0967);
\coordinate (s544) at (-0.3519,0.1204,0.0203);
\coordinate (s545) at (0.4599,-0.1843,-0.0218);
\coordinate (s546) at (0.0907,-0.0864,0.2568);
\coordinate (s547) at (0.3665,-0.1759,0.1075);
\coordinate (s548) at (-0.2971,0.1676,-0.0757);
\coordinate (s549) at (-0.1270,0.0904,0.1483);
\coordinate (s550) at (-0.3220,0.0591,0.0485);
\coordinate (s551) at (-0.1786,-0.3089,0.1888);
\coordinate (s552) at (-0.0933,0.3494,-0.0169);
\coordinate (s553) at (0.2854,-0.2577,-0.1069);
\coordinate (s554) at (-0.3420,0.1266,-0.0161);
\coordinate (s555) at (0.0215,0.1076,0.1478);
\coordinate (s556) at (-0.2607,0.4021,-0.2032);
\coordinate (s557) at (-0.1890,0.3034,-0.1246);
\coordinate (s558) at (0.0915,-0.3145,-0.1816);
\coordinate (s559) at (-0.2048,-0.2808,0.0202);
\coordinate (s560) at (-0.2892,0.0033,0.1281);
\coordinate (s561) at (-0.1947,0.4035,-0.3773);
\coordinate (s562) at (-0.0596,-0.2283,-0.1094);
\coordinate (s563) at (-0.1581,0.1752,0.1576);
\coordinate (s564) at (-0.2162,0.4165,-0.2658);
\coordinate (s565) at (0.0892,0.1196,0.1599);
\coordinate (s566) at (-0.1584,0.0618,-0.1499);
\coordinate (s567) at (-0.1172,0.1392,-0.1230);
\coordinate (s568) at (0.2279,0.1222,0.1434);
\coordinate (s569) at (0.2878,-0.1107,0.1847);
\coordinate (s570) at (-0.2301,0.4657,-0.3364);
\coordinate (s571) at (0.0400,-0.3140,-0.1984);
\coordinate (s572) at (-0.2417,0.1040,-0.0955);
\coordinate (s573) at (-0.1874,-0.3023,0.1835);
\coordinate (s574) at (0.2044,-0.3154,0.1649);
\coordinate (s575) at (0.2881,-0.0864,-0.1770);
\coordinate (s576) at (-0.3358,0.2266,0.1423);
\coordinate (s577) at (-0.1264,0.2286,0.0762);
\coordinate (s578) at (-0.3125,0.2404,0.1837);
\coordinate (s579) at (-0.2475,0.3335,0.0147);
\coordinate (s580) at (0.0866,-0.1295,0.2443);
\coordinate (s581) at (0.0616,0.1881,0.0122);
\coordinate (s582) at (-0.0137,-0.1809,-0.1720);
\coordinate (s583) at (0.0074,-0.2998,-0.1494);
\coordinate (s584) at (-0.3439,0.1490,-0.0138);
\coordinate (s585) at (-0.2903,0.2798,0.1647);
\coordinate (s586) at (-0.0189,-0.3068,0.0813);
\coordinate (s587) at (0.4064,-0.2541,-0.0445);
\coordinate (s588) at (-0.0633,-0.3177,0.0960);
\coordinate (s589) at (0.2881,-0.0656,-0.1748);
\coordinate (s590) at (0.3370,-0.0150,-0.1322);
\coordinate (s591) at (-0.1927,-0.2776,0.0880);
\coordinate (s592) at (-0.2967,0.0868,-0.0503);
\coordinate (s593) at (0.0232,-0.1321,0.2081);
\coordinate (s594) at (0.0888,-0.2938,-0.0512);
\coordinate (s595) at (0.0019,-0.1302,0.1705);
\coordinate (s596) at (-0.1339,-0.1031,0.1740);
\coordinate (s597) at (-0.0410,-0.0311,0.1783);
\coordinate (s598) at (-0.2041,-0.0934,-0.1427);
\coordinate (s599) at (-0.0675,0.3132,-0.0294);
\coordinate (s600) at (-0.1682,0.2237,-0.0830);
\coordinate (s601) at (0.1279,-0.2944,0.0645);
\coordinate (s602) at (0.2748,-0.2140,0.1726);
\coordinate (s603) at (0.0671,0.1388,-0.1181);
\coordinate (s604) at (-0.2540,0.3154,-0.1913);
\coordinate (s605) at (0.0315,0.0532,-0.1753);
\coordinate (s606) at (-0.2249,0.4674,-0.3472);
\coordinate (s607) at (-0.2399,0.3725,-0.2821);
\coordinate (s608) at (-0.0611,0.0156,-0.1715);
\coordinate (s609) at (0.0301,0.1784,-0.0101);
\coordinate (s610) at (0.0504,0.5000,-0.1574);
\coordinate (s611) at (-0.1652,-0.3149,0.1839);
\coordinate (s612) at (0.2363,-0.2481,0.1778);
\coordinate (s613) at (0.0615,-0.0864,0.2504);
\coordinate (s614) at (0.1263,0.1927,-0.0482);
\coordinate (s615) at (-0.3521,0.1625,0.1536);
\coordinate (s616) at (-0.3610,0.1693,0.0565);
\coordinate (s617) at (0.2226,0.0644,0.1808);
\coordinate (s618) at (0.1254,0.1998,-0.0020);
\coordinate (s619) at (-0.0489,0.0622,-0.1605);
\coordinate (s620) at (0.4641,-0.1419,0.0452);
\coordinate (s621) at (-0.1035,0.3591,-0.0947);
\coordinate (s622) at (0.0951,-0.2953,0.0152);
\coordinate (s623) at (0.0794,-0.3180,-0.1567);
\coordinate (s624) at (0.1856,-0.3099,-0.0213);
\coordinate (s625) at (-0.1264,-0.2459,0.0436);
\coordinate (s626) at (0.1324,0.0146,-0.2165);
\coordinate (s627) at (0.1207,0.1260,-0.1341);
\coordinate (s628) at (0.4181,-0.1727,-0.0699);
\coordinate (s629) at (-0.1597,-0.1810,-0.0648);
\coordinate (s630) at (0.2449,-0.1086,-0.2029);
\coordinate (s631) at (-0.1326,-0.2311,0.1255);
\coordinate (s632) at (-0.1486,-0.1864,-0.0850);
\coordinate (s633) at (-0.2661,0.3521,-0.1885);
\coordinate (s634) at (0.0998,-0.2935,-0.0538);
\coordinate (s635) at (-0.2711,0.3398,-0.1551);
\coordinate (s636) at (0.1600,-0.2184,-0.2119);
\coordinate (s637) at (-0.1152,0.2151,0.0738);
\coordinate (s638) at (-0.1542,-0.3209,-0.1015);
\coordinate (s639) at (-0.2922,0.2637,0.1801);
\coordinate (s640) at (-0.0653,0.4306,-0.0794);
\coordinate (s641) at (-0.0434,0.3575,-0.1228);
\coordinate (s642) at (0.3643,-0.0418,-0.1035);
\coordinate (s643) at (0.3912,-0.2698,-0.0341);
\coordinate (s644) at (-0.3086,-0.0841,0.0297);
\coordinate (s645) at (-0.2766,-0.1243,-0.0127);
\coordinate (s646) at (-0.2900,0.3265,0.0570);
\coordinate (s647) at (0.4272,-0.1116,-0.0064);
\coordinate (s648) at (-0.2689,0.2479,-0.0809);
\coordinate (s649) at (0.2878,-0.3090,0.0621);
\coordinate (s650) at (-0.2813,0.1003,-0.0634);
\coordinate (s651) at (0.2790,-0.0856,0.2046);
\coordinate (s652) at (0.2334,-0.2928,-0.1594);
\coordinate (s653) at (0.1115,-0.1121,-0.2452);
\coordinate (s654) at (0.0665,0.4762,-0.1986);
\coordinate (s655) at (0.4419,-0.2252,0.0655);
\coordinate (s656) at (0.1910,0.0894,-0.1558);
\coordinate (s657) at (-0.1292,-0.1979,0.1150);
\coordinate (s658) at (0.2132,0.1212,0.1456);
\coordinate (s659) at (-0.2474,0.3721,-0.1263);
\coordinate (s660) at (0.3371,0.0591,0.1089);
\coordinate (s661) at (0.1413,0.0392,0.1919);
\coordinate (s662) at (-0.1621,0.3288,0.0348);
\coordinate (s663) at (-0.3291,0.1071,-0.0190);
\coordinate (s664) at (-0.1487,0.2764,-0.0587);
\coordinate (s665) at (-0.0927,0.2983,-0.0152);
\coordinate (s666) at (-0.2522,0.3989,-0.2833);
\coordinate (s667) at (0.3739,0.0118,0.0732);
\coordinate (s668) at (0.2232,0.1536,-0.0999);
\coordinate (s669) at (0.1512,-0.1498,-0.2343);
\coordinate (s670) at (-0.1654,-0.2453,0.1527);
\coordinate (s671) at (0.0673,0.1862,-0.0256);
\coordinate (s672) at (-0.0747,-0.3160,0.1337);
\coordinate (s673) at (0.2466,-0.3108,-0.0214);
\coordinate (s674) at (0.0999,-0.3151,0.1835);
\coordinate (s675) at (-0.0583,-0.2702,-0.1938);
\coordinate (s676) at (0.0537,0.0853,0.1695);
\coordinate (s677) at (-0.0630,0.3873,-0.0380);
\coordinate (s678) at (0.1188,-0.0747,-0.2508);
\coordinate (s679) at (0.3781,-0.1607,-0.0608);
\coordinate (s680) at (0.0699,0.4699,-0.1728);
\coordinate (s681) at (0.1169,-0.1094,-0.2447);
\coordinate (s682) at (0.3759,-0.1009,0.0915);
\coordinate (s683) at (0.3178,-0.2997,-0.0442);
\coordinate (s684) at (0.3159,-0.0941,0.1731);
\coordinate (s685) at (-0.0694,-0.1351,-0.1355);
\coordinate (s686) at (0.3565,-0.1006,-0.1023);
\coordinate (s687) at (-0.2925,0.1705,0.2262);
\coordinate (s688) at (-0.1472,0.2543,0.1017);
\coordinate (s689) at (0.3278,0.1071,0.0734);
\coordinate (s690) at (-0.0029,-0.3171,-0.1628);
\coordinate (s691) at (0.4093,-0.2600,-0.0279);
\coordinate (s692) at (-0.2220,0.3539,-0.0994);
\coordinate (s693) at (0.0223,-0.2306,0.1907);
\coordinate (s694) at (0.3956,-0.2518,-0.0579);
\coordinate (s695) at (0.3995,-0.2169,-0.0782);
\coordinate (s696) at (0.0592,0.4204,-0.1795);
\coordinate (s697) at (-0.0896,-0.3087,-0.1889);
\coordinate (s698) at (0.2866,-0.2917,0.1050);
\coordinate (s699) at (0.0425,0.0816,0.1694);
\coordinate (s700) at (-0.0928,0.4075,-0.0853);
\coordinate (s701) at (-0.1856,0.1928,0.1639);
\coordinate (s702) at (0.3211,-0.1546,0.1623);
\coordinate (s703) at (-0.1746,-0.2665,-0.0828);
\coordinate (s704) at (0.3891,-0.0341,-0.0054);
\coordinate (s705) at (-0.0073,-0.2854,0.2347);
\coordinate (s706) at (-0.0296,-0.1858,-0.1195);
\coordinate (s707) at (0.0718,-0.2428,-0.2135);
\coordinate (s708) at (0.3611,-0.0937,-0.0950);
\coordinate (s709) at (-0.0812,0.1754,-0.0807);
\coordinate (s710) at (0.0159,0.0090,-0.1941);
\coordinate (s711) at (-0.0758,-0.1861,0.1641);
\coordinate (s712) at (-0.0022,-0.1326,-0.2283);
\coordinate (s713) at (-0.1930,-0.2966,0.0776);
\coordinate (s714) at (-0.0538,0.1816,-0.0305);
\coordinate (s715) at (0.1665,0.1135,0.1645);
\coordinate (s716) at (-0.3569,0.1385,0.0760);
\coordinate (s717) at (-0.1024,-0.2806,-0.1256);
\coordinate (s718) at (0.2858,-0.2773,0.1292);
\coordinate (s719) at (-0.2212,0.0313,0.1688);
\coordinate (s720) at (0.2215,-0.0511,-0.2111);
\coordinate (s721) at (0.1261,-0.2605,-0.1982);
\coordinate (s722) at (-0.1439,0.1038,0.1385);
\coordinate (s723) at (0.2051,-0.1980,-0.2103);
\coordinate (s724) at (-0.2461,0.4529,-0.3068);
\coordinate (s725) at (-0.2835,-0.0529,0.1320);
\coordinate (s726) at (-0.0700,-0.0172,-0.1755);
\coordinate (s727) at (-0.2122,-0.0849,-0.1426);
\coordinate (s728) at (-0.1326,0.0104,0.1834);
\coordinate (s729) at (-0.0681,-0.3196,-0.0091);
\coordinate (s730) at (0.3899,-0.1429,0.0901);
\coordinate (s731) at (-0.0849,-0.2573,-0.1289);
\coordinate (s732) at (0.1264,0.0298,0.2171);
\coordinate (s733) at (-0.1989,-0.2581,-0.0465);
\coordinate (s734) at (-0.1987,0.3931,-0.2456);
\coordinate (s735) at (-0.1904,0.1274,0.1755);
\coordinate (s736) at (0.3552,-0.1577,-0.0954);
\coordinate (s737) at (-0.1809,-0.2999,0.1889);
\coordinate (s738) at (-0.0641,-0.3132,0.1728);
\coordinate (s739) at (-0.0231,0.1184,0.1246);
\coordinate (s740) at (0.3976,-0.2256,-0.0764);
\coordinate (s741) at (-0.3444,0.2490,0.0495);
\coordinate (s742) at (-0.1640,-0.2444,0.1234);
\coordinate (s743) at (0.3590,-0.1653,-0.0793);
\coordinate (s744) at (0.1016,-0.3148,0.1955);
\coordinate (s745) at (-0.2244,0.1061,-0.1037);
\coordinate (s746) at (0.1481,0.0694,0.1784);
\coordinate (s747) at (-0.1373,-0.1907,0.0768);
\coordinate (s748) at (-0.0621,-0.3143,0.0009);
\coordinate (s749) at (-0.1635,-0.2722,0.1908);
\coordinate (s750) at (-0.1182,0.3682,-0.0192);
\coordinate (s751) at (-0.3128,0.2641,-0.0146);
\coordinate (s752) at (0.2124,0.0127,-0.1840);
\coordinate (s753) at (0.1228,0.1961,-0.0320);
\coordinate (s754) at (0.1721,-0.1262,-0.2309);
\coordinate (s755) at (-0.0129,-0.2246,-0.1651);
\coordinate (s756) at (-0.0181,0.1694,0.0416);
\coordinate (s757) at (0.0434,0.0896,0.1656);
\coordinate (s758) at (-0.0505,0.3967,-0.0498);
\coordinate (s759) at (-0.3092,-0.0155,-0.0715);
\coordinate (s760) at (-0.1019,0.1231,-0.1340);
\coordinate (s761) at (0.0445,-0.0222,0.2457);
\coordinate (s762) at (-0.1331,-0.2201,0.0730);
\coordinate (s763) at (0.2730,-0.1928,-0.1838);
\coordinate (s764) at (-0.1964,0.2903,0.1516);
\coordinate (s765) at (0.0744,0.1402,0.1427);
\coordinate (s766) at (0.0214,0.1517,0.0983);
\coordinate (s767) at (0.2322,0.0940,0.1567);
\coordinate (s768) at (0.4285,-0.1488,-0.0514);
\coordinate (s769) at (0.2333,-0.0328,-0.2032);
\coordinate (s770) at (0.3658,0.0554,-0.0130);
\coordinate (s771) at (-0.2235,0.3567,-0.1025);
\coordinate (s772) at (0.0703,0.1270,0.1507);
\coordinate (s773) at (-0.2270,-0.1290,-0.0872);
\coordinate (s774) at (-0.2713,0.0818,0.1581);
\coordinate (s775) at (-0.3346,0.0195,0.0359);
\coordinate (s776) at (-0.2096,-0.2672,0.0006);
\coordinate (s777) at (0.3023,-0.0963,0.1824);
\coordinate (s778) at (0.2618,-0.0483,-0.1902);
\coordinate (s779) at (-0.2529,0.4315,-0.2656);
\coordinate (s780) at (0.3473,-0.2925,0.0553);
\coordinate (s781) at (0.0839,-0.1429,0.2411);
\coordinate (s782) at (-0.2625,0.3287,0.0868);
\coordinate (s783) at (0.0920,0.4481,-0.1948);
\coordinate (s784) at (-0.2498,0.1438,-0.0942);
\coordinate (s785) at (0.3427,0.0248,-0.1051);
\coordinate (s786) at (0.2252,-0.2948,-0.1643);
\coordinate (s787) at (0.0579,-0.1039,0.2457);
\coordinate (s788) at (-0.1333,0.3521,-0.0084);
\coordinate (s789) at (-0.2570,0.3145,-0.1536);
\coordinate (s790) at (-0.3195,-0.0497,-0.0081);
\coordinate (s791) at (-0.0346,-0.0578,-0.1916);
\coordinate (s792) at (-0.2006,0.4021,-0.2716);
\coordinate (s793) at (-0.1875,0.4376,-0.3582);
\coordinate (s794) at (0.0850,-0.2510,-0.2093);
\coordinate (s795) at (-0.0359,-0.3199,-0.0055);
\coordinate (s796) at (-0.3362,0.2134,0.1554);
\coordinate (s797) at (0.0568,-0.3165,-0.1878);
\coordinate (s798) at (0.0444,0.1257,0.1426);
\coordinate (s799) at (0.2747,0.0663,0.1578);
\coordinate (s800) at (0.2706,-0.1898,-0.1862);
\coordinate (s801) at (0.0847,-0.2951,0.0684);
\coordinate (s802) at (0.1521,0.0935,0.1753);
\coordinate (s803) at (-0.0775,-0.0760,-0.1563);
\coordinate (s804) at (-0.0923,0.0432,0.1730);
\coordinate (s805) at (0.2904,-0.0845,0.1931);
\coordinate (s806) at (0.0633,-0.1590,-0.2498);
\coordinate (s807) at (0.4038,-0.2072,0.1134);
\coordinate (s808) at (0.2821,-0.2427,0.1538);
\coordinate (s809) at (-0.2047,-0.0275,0.1873);
\coordinate (s810) at (-0.1008,0.3828,-0.0924);
\coordinate (s811) at (0.4485,-0.1194,-0.0080);
\coordinate (s812) at (0.0875,0.0196,0.2269);
\coordinate (s813) at (0.1923,-0.3162,-0.0739);
\coordinate (s814) at (0.0034,0.4512,-0.1480);
\coordinate (s815) at (0.3656,0.0181,-0.0698);
\coordinate (s816) at (0.2021,-0.3131,0.1335);
\coordinate (s817) at (0.4041,-0.2691,-0.0028);
\coordinate (s818) at (-0.3107,0.0512,0.0882);
\coordinate (s819) at (-0.2513,0.1866,0.2292);
\coordinate (s820) at (0.0103,0.1545,-0.0824);
\coordinate (s821) at (0.0285,-0.1852,-0.2286);
\coordinate (s822) at (0.1642,0.0182,0.2258);
\coordinate (s823) at (-0.0296,-0.1898,-0.1181);
\coordinate (s824) at (-0.1415,-0.2558,-0.0910);
\coordinate (s825) at (0.0354,-0.2962,0.0736);
\coordinate (s826) at (-0.0374,-0.0613,-0.1850);
\coordinate (s827) at (0.1221,-0.3104,0.2027);
\coordinate (s828) at (-0.1283,-0.2409,0.0326);
\coordinate (s829) at (0.2504,-0.0079,0.2041);
\coordinate (s830) at (-0.1422,0.3616,-0.0233);
\coordinate (s831) at (-0.0087,0.1567,-0.0749);
\coordinate (s832) at (-0.2208,-0.3209,-0.0401);
\coordinate (s833) at (0.2955,-0.1296,-0.1696);
\coordinate (s834) at (0.1332,-0.2919,0.1101);
\coordinate (s835) at (-0.2701,0.3285,0.0005);
\coordinate (s836) at (0.2684,-0.1990,-0.1872);
\coordinate (s837) at (-0.1198,-0.2464,-0.0998);
\coordinate (s838) at (-0.0640,-0.2442,-0.1258);
\coordinate (s839) at (0.4259,-0.2172,0.0929);
\coordinate (s840) at (-0.2145,-0.1448,0.1090);
\coordinate (s841) at (-0.2699,0.3866,-0.2491);
\coordinate (s842) at (0.0144,0.4424,-0.1588);
\coordinate (s843) at (0.0097,-0.1501,0.1729);
\coordinate (s844) at (-0.2689,-0.1155,-0.0643);
\coordinate (s845) at (0.2193,-0.3141,0.1587);
\coordinate (s846) at (-0.1375,0.0539,-0.1585);
\coordinate (s847) at (0.1190,0.0448,0.1832);
\coordinate (s848) at (-0.0784,-0.2689,-0.1717);
\coordinate (s849) at (0.0910,0.1527,-0.1085);
\coordinate (s850) at (-0.1122,0.2276,0.0136);
\coordinate (s851) at (-0.2259,-0.2894,-0.0588);
\coordinate (s852) at (0.2000,-0.2150,-0.2090);
\coordinate (s853) at (0.2146,0.1288,0.1427);
\coordinate (s854) at (0.0265,0.1742,-0.0321);
\coordinate (s855) at (0.4031,-0.2693,0.0345);
\coordinate (s856) at (-0.0879,-0.1929,-0.1143);
\coordinate (s857) at (-0.2385,-0.0609,0.1632);
\coordinate (s858) at (0.0267,0.1609,0.0794);
\coordinate (s859) at (-0.2700,0.3085,0.1370);
\coordinate (s860) at (0.0168,-0.2956,-0.0676);
\coordinate (s861) at (-0.1897,0.3765,-0.3017);
\coordinate (s862) at (-0.3425,0.1174,0.0800);
\coordinate (s863) at (0.0177,-0.0694,-0.2556);
\coordinate (s864) at (-0.1119,0.3277,-0.0864);
\coordinate (s865) at (0.1432,-0.3130,-0.0054);
\coordinate (s866) at (0.3333,-0.2307,0.1171);
\coordinate (s867) at (-0.0943,0.1478,-0.1175);
\coordinate (s868) at (0.4439,-0.1218,0.0600);
\coordinate (s869) at (-0.3122,0.0634,0.0714);
\coordinate (s870) at (-0.1620,0.2082,-0.0832);
\coordinate (s871) at (0.3080,0.1362,0.0248);
\coordinate (s872) at (0.1585,-0.2923,-0.1103);
\coordinate (s873) at (0.0861,0.4654,-0.1965);
\coordinate (s874) at (0.0901,-0.0530,-0.2559);
\coordinate (s875) at (-0.2872,0.3255,0.0110);
\coordinate (s876) at (0.1009,-0.1788,0.2448);
\coordinate (s877) at (0.1833,-0.3149,0.1736);
\coordinate (s878) at (-0.1893,0.3588,-0.2688);
\coordinate (s879) at (-0.2007,0.0494,-0.1430);
\coordinate (s880) at (-0.1013,-0.2537,-0.1070);
\coordinate (s881) at (0.2498,-0.3011,-0.0937);
\coordinate (s882) at (0.3573,-0.1434,-0.0984);
\coordinate (s883) at (-0.2157,-0.0232,0.1824);
\coordinate (s884) at (-0.1827,-0.3210,-0.0898);
\coordinate (s885) at (-0.0926,0.0546,-0.1636);
\coordinate (s886) at (0.2796,-0.0191,0.1984);
\coordinate (s887) at (-0.0782,0.2943,-0.0672);
\coordinate (s888) at (0.1996,-0.3156,0.0677);
\coordinate (s889) at (-0.2551,0.1740,-0.0951);
\coordinate (s890) at (0.1486,0.0490,0.1839);
\coordinate (s891) at (0.0011,0.1669,0.0459);
\coordinate (s892) at (0.0458,0.0216,0.1962);
\coordinate (s893) at (-0.1716,-0.1002,-0.1473);
\coordinate (s894) at (-0.2629,0.2311,0.2161);
\coordinate (s895) at (0.1188,-0.2701,-0.1891);
\coordinate (s896) at (0.0634,-0.1689,-0.2458);
\coordinate (s897) at (-0.3010,-0.0763,-0.0430);
\coordinate (s898) at (-0.1075,-0.2459,0.1612);
\coordinate (s899) at (-0.3067,-0.0611,0.0833);
\coordinate (s900) at (0.0250,-0.2965,0.0113);
\coordinate (s901) at (-0.0433,0.1451,0.1019);
\coordinate (s902) at (0.1316,0.1952,-0.0409);
\coordinate (s903) at (-0.2469,-0.0569,0.1594);
\coordinate (s904) at (-0.1599,-0.1780,-0.0675);
\coordinate (s905) at (0.0937,-0.2164,-0.2290);
\coordinate (s906) at (-0.1610,-0.1522,-0.0975);
\coordinate (s907) at (-0.3353,-0.0077,0.0363);
\coordinate (s908) at (0.0804,0.4510,-0.1771);
\coordinate (s909) at (0.0370,0.1107,0.1512);
\coordinate (s910) at (0.1927,-0.2765,0.1900);
\coordinate (s911) at (-0.1262,0.2028,-0.0623);
\coordinate (s912) at (-0.2361,0.3324,-0.0000);
\coordinate (s913) at (0.3795,0.0060,-0.0410);
\coordinate (s914) at (0.1153,0.0705,-0.1720);
\coordinate (s915) at (0.2300,0.1884,0.0159);
\coordinate (s916) at (-0.2637,-0.1120,0.1045);
\coordinate (s917) at (0.2509,0.0418,-0.1650);
\coordinate (s918) at (-0.0094,0.1422,0.0967);
\coordinate (s919) at (-0.2258,0.3219,-0.3175);
\coordinate (s920) at (0.2606,-0.0933,-0.1929);
\coordinate (s921) at (-0.1527,-0.2934,-0.1068);
\coordinate (s922) at (0.2688,0.1674,-0.0046);
\coordinate (s923) at (-0.2284,0.3705,-0.3176);
\coordinate (s924) at (-0.2144,0.1257,-0.0994);
\coordinate (s925) at (-0.0240,0.1086,-0.1409);
\coordinate (s926) at (-0.0262,-0.0173,-0.1834);
\coordinate (s927) at (-0.0443,-0.2044,-0.1079);
\coordinate (s928) at (0.3746,-0.1880,-0.0777);
\coordinate (s929) at (0.0160,-0.1377,0.1915);
\coordinate (s930) at (-0.1976,0.3940,-0.3746);
\coordinate (s931) at (0.4218,-0.1238,0.0751);
\coordinate (s932) at (-0.2083,-0.3007,0.0977);
\coordinate (s933) at (-0.1387,0.1435,-0.1136);
\coordinate (s934) at (0.0298,-0.0842,0.2418);
\coordinate (s935) at (-0.1248,-0.2202,0.1289);
\coordinate (s936) at (-0.2259,0.3264,0.1078);
\coordinate (s937) at (0.3305,-0.2936,0.0716);
\coordinate (s938) at (0.4255,-0.2164,0.0938);
\coordinate (s939) at (0.1678,0.0291,0.2076);
\coordinate (s940) at (0.0628,-0.2931,-0.0954);
\coordinate (s941) at (0.0938,-0.2950,-0.0070);
\coordinate (s942) at (-0.1428,0.2752,0.0782);
\coordinate (s943) at (0.1600,-0.2955,-0.1201);
\coordinate (s944) at (-0.0144,0.3359,-0.1049);
\coordinate (s945) at (0.2063,-0.3179,-0.0509);
\coordinate (s946) at (0.3291,0.1076,-0.0381);
\coordinate (s947) at (-0.0972,-0.3155,0.1561);
\coordinate (s948) at (-0.0040,-0.0977,-0.2420);
\coordinate (s949) at (0.1816,-0.0547,-0.2284);
\coordinate (s950) at (0.4216,-0.1890,0.1064);
\coordinate (s951) at (0.2834,0.1556,-0.0155);
\coordinate (s952) at (-0.0330,-0.2959,-0.0593);
\coordinate (s953) at (-0.1223,-0.1848,0.1290);
\coordinate (s954) at (0.1495,-0.3163,0.0064);
\coordinate (s955) at (0.2553,0.1755,-0.0011);
\coordinate (s956) at (-0.1069,-0.1052,0.1730);
\coordinate (s957) at (-0.1091,-0.0835,0.1802);
\coordinate (s958) at (0.3565,0.0724,0.0129);
\coordinate (s959) at (-0.1943,0.3296,0.0897);
\coordinate (s960) at (-0.1916,-0.3166,0.1286);
\coordinate (s961) at (0.2851,-0.0777,-0.1786);
\coordinate (s962) at (0.0958,-0.1731,-0.2388);
\coordinate (s963) at (-0.0250,-0.2940,-0.1340);
\coordinate (s964) at (-0.1563,0.2994,0.1094);
\coordinate (s965) at (-0.1825,-0.3209,-0.0942);
\coordinate (s966) at (0.3847,-0.0262,0.0492);
\coordinate (s967) at (0.2692,-0.2641,0.1636);
\coordinate (s968) at (-0.2037,-0.2929,0.1573);
\coordinate (s969) at (-0.2906,-0.1051,-0.0339);
\coordinate (s970) at (-0.0306,-0.3140,0.0925);
\coordinate (s971) at (-0.1022,-0.2838,-0.1313);
\coordinate (s972) at (-0.1231,-0.0175,0.1871);
\coordinate (s973) at (0.4572,-0.2079,0.0444);
\coordinate (s974) at (-0.1509,-0.0250,-0.1690);
\coordinate (s975) at (-0.0744,-0.1887,0.1639);
\coordinate (s976) at (0.3342,-0.1202,0.1512);
\coordinate (s977) at (-0.3456,0.1830,0.1535);
\coordinate (s978) at (0.3561,-0.2762,0.0882);
\coordinate (s979) at (-0.2961,0.2161,-0.0645);
\coordinate (s980) at (-0.1771,-0.3064,-0.1018);
\coordinate (s981) at (-0.2874,0.1844,0.2306);
\coordinate (s982) at (-0.2942,0.2164,0.2161);
\coordinate (s983) at (0.3639,-0.1419,0.1047);
\coordinate (s984) at (-0.2301,0.1054,0.2123);
\coordinate (s985) at (-0.0728,0.1766,-0.0721);
\coordinate (s986) at (-0.1271,-0.0290,0.1912);
\coordinate (s987) at (0.3256,0.0964,-0.0703);
\coordinate (s988) at (-0.1621,-0.0747,-0.1593);
\coordinate (s989) at (0.2338,0.0294,0.2000);
\coordinate (s990) at (0.0353,-0.3205,-0.1732);
\coordinate (s991) at (-0.0307,0.3498,-0.1197);
\coordinate (s992) at (-0.3275,0.1412,-0.0462);
\coordinate (s993) at (-0.2889,0.1716,0.2281);
\coordinate (s994) at (0.0027,0.0986,0.1445);
\coordinate (s995) at (-0.2411,-0.0989,0.1429);
\coordinate (s996) at (0.1709,0.1572,0.1324);
\coordinate (s997) at (0.0725,-0.2953,0.0722);
\coordinate (s998) at (-0.2655,-0.1360,0.0258);
\coordinate (s999) at (0.3799,-0.0618,0.0837);

% Target point cloud
\coordinate (t0) at (2.0655,0.2094,0.3689);
\coordinate (t1) at (2.3846,0.3635,0.2284);
\coordinate (t2) at (2.0907,0.7157,0.1768);
\coordinate (t3) at (2.2057,0.3014,0.0315);
\coordinate (t4) at (1.8816,0.9121,0.3068);
\coordinate (t5) at (1.7792,0.7076,0.5733);
\coordinate (t6) at (2.4684,0.4813,0.1514);
\coordinate (t7) at (1.9534,0.3804,0.0699);
\coordinate (t8) at (2.2474,0.6857,0.1343);
\coordinate (t9) at (1.8342,0.7274,0.3963);
\coordinate (t10) at (2.1744,0.7024,0.1456);
\coordinate (t11) at (1.7302,0.7526,0.3767);
\coordinate (t12) at (1.7552,0.6618,0.3540);
\coordinate (t13) at (1.7457,0.4658,0.5218);
\coordinate (t14) at (1.9423,0.5092,0.4980);
\coordinate (t15) at (2.1152,0.2561,0.1581);
\coordinate (t16) at (2.2635,0.2186,0.2751);
\coordinate (t17) at (1.8540,0.6272,0.5504);
\coordinate (t18) at (1.6672,0.6799,0.5487);
\coordinate (t19) at (1.6610,0.6691,0.4809);
\coordinate (t20) at (2.2282,0.4226,-0.0138);
\coordinate (t21) at (2.2650,0.3774,0.0283);
\coordinate (t22) at (1.8795,0.2695,0.3920);
\coordinate (t23) at (2.2767,0.4091,0.0255);
\coordinate (t24) at (1.9031,0.4894,0.1012);
\coordinate (t25) at (2.3956,0.3987,0.2258);
\coordinate (t26) at (1.9462,0.2063,0.3264);
\coordinate (t27) at (1.9147,0.1765,0.2919);
\coordinate (t28) at (1.8999,1.0087,0.3188);
\coordinate (t29) at (2.0285,0.4731,0.0035);
\coordinate (t30) at (2.4667,0.4289,0.1731);
\coordinate (t31) at (1.8513,0.9312,0.3427);
\coordinate (t32) at (1.9344,0.1124,0.3918);
\coordinate (t33) at (1.6511,0.5861,0.4534);
\coordinate (t34) at (1.9615,0.3226,0.0728);
\coordinate (t35) at (1.8733,0.2828,0.2198);
\coordinate (t36) at (2.3387,0.4242,0.3683);
\coordinate (t37) at (2.1193,0.3332,0.4253);
\coordinate (t38) at (1.8798,0.9886,0.3094);
\coordinate (t39) at (2.0918,0.1539,0.3492);
\coordinate (t40) at (2.1811,0.1667,0.3680);
\coordinate (t41) at (2.4488,0.3894,0.1844);
\coordinate (t42) at (1.9473,0.2089,0.3147);
\coordinate (t43) at (1.7035,0.7522,0.3177);
\coordinate (t44) at (1.9583,0.2005,0.3714);
\coordinate (t45) at (1.7508,0.5704,0.3070);
\coordinate (t46) at (1.6662,0.5038,0.4797);
\coordinate (t47) at (2.2616,0.6397,0.3895);
\coordinate (t48) at (1.8912,0.2664,0.3645);
\coordinate (t49) at (1.6663,0.6035,0.3968);
\coordinate (t50) at (1.8526,0.3216,0.2167);
\coordinate (t51) at (1.8826,0.9774,0.3690);
\coordinate (t52) at (1.8944,0.9129,0.3418);
\coordinate (t53) at (1.9493,0.2205,0.3150);
\coordinate (t54) at (1.8310,0.4571,0.5661);
\coordinate (t55) at (2.2042,0.4040,-0.0157);
\coordinate (t56) at (2.4242,0.3538,0.1334);
\coordinate (t57) at (1.9022,0.4782,0.5161);
\coordinate (t58) at (2.3361,0.3139,0.3058);
\coordinate (t59) at (1.8993,0.1753,0.1810);
\coordinate (t60) at (1.6678,0.6657,0.4396);
\coordinate (t61) at (1.7991,0.3477,0.2192);
\coordinate (t62) at (1.9393,0.1642,0.4008);
\coordinate (t63) at (2.1201,0.7460,0.2838);
\coordinate (t64) at (1.6986,0.5929,0.5958);
\coordinate (t65) at (1.7650,0.6565,0.6216);
\coordinate (t66) at (2.3729,0.4006,0.2961);
\coordinate (t67) at (2.3121,0.3574,0.3759);
\coordinate (t68) at (2.0570,0.3116,-0.0008);
\coordinate (t69) at (2.4654,0.4758,0.1197);
\coordinate (t70) at (1.9625,0.1452,0.2932);
\coordinate (t71) at (1.6929,0.4437,0.3485);
\coordinate (t72) at (2.3374,0.6391,0.2038);
\coordinate (t73) at (2.3974,0.4359,0.2244);
\coordinate (t74) at (1.8497,0.4242,0.1720);
\coordinate (t75) at (1.8770,0.1582,0.2813);
\coordinate (t76) at (2.1104,0.6807,0.4138);
\coordinate (t77) at (2.1659,0.6800,0.4113);
\coordinate (t78) at (2.1221,0.1812,0.4011);
\coordinate (t79) at (2.4724,0.4502,0.1521);
\coordinate (t80) at (1.9589,0.3908,0.0405);
\coordinate (t81) at (1.7355,0.5091,0.2751);
\coordinate (t82) at (2.0966,0.7401,0.2454);
\coordinate (t83) at (1.6945,0.4827,0.3839);
\coordinate (t84) at (2.0504,0.7034,0.3501);
\coordinate (t85) at (2.4582,0.4012,0.1216);
\coordinate (t86) at (2.0408,0.2856,0.4087);
\coordinate (t87) at (2.1676,0.3284,0.4437);
\coordinate (t88) at (2.2893,0.4579,0.4271);
\coordinate (t89) at (1.9686,0.5126,0.4903);
\coordinate (t90) at (2.0996,0.2648,0.3564);
\coordinate (t91) at (2.0195,0.1311,0.3691);
\coordinate (t92) at (1.7890,0.7225,0.5499);
\coordinate (t93) at (2.2598,0.4433,0.4553);
\coordinate (t94) at (2.1825,0.5845,0.4444);
\coordinate (t95) at (2.2122,0.2532,0.2197);
\coordinate (t96) at (1.9066,0.4723,0.1200);
\coordinate (t97) at (1.6666,0.6924,0.5224);
\coordinate (t98) at (1.6536,0.7659,0.2660);
\coordinate (t99) at (1.7767,0.6788,0.6051);
\coordinate (t100) at (1.6682,0.7609,0.4238);
\coordinate (t101) at (2.1579,0.3942,0.4883);
\coordinate (t102) at (1.6702,0.6642,0.4210);
\coordinate (t103) at (2.3594,0.6076,0.2692);
\coordinate (t104) at (1.7555,0.4616,0.6173);
\coordinate (t105) at (2.0992,0.3613,-0.0099);
\coordinate (t106) at (1.9549,0.3668,0.1226);
\coordinate (t107) at (2.2849,0.3296,0.4009);
\coordinate (t108) at (1.9719,0.4308,0.4977);
\coordinate (t109) at (1.9517,0.5520,0.0449);
\coordinate (t110) at (1.8738,0.5470,0.5695);
\coordinate (t111) at (2.2586,0.6136,0.3983);
\coordinate (t112) at (2.3108,0.3449,0.0450);
\coordinate (t113) at (2.0895,0.3058,-0.0094);
\coordinate (t114) at (1.7333,0.3421,0.4010);
\coordinate (t115) at (1.8636,0.3069,0.2225);
\coordinate (t116) at (1.9605,0.2762,0.0074);
\coordinate (t117) at (2.2522,0.4175,0.4504);
\coordinate (t118) at (2.1910,0.5802,0.4399);
\coordinate (t119) at (1.9631,0.1101,0.4042);
\coordinate (t120) at (1.7910,0.2913,0.3413);
\coordinate (t121) at (1.8537,0.3245,0.2141);
\coordinate (t122) at (2.4514,0.4122,0.0963);
\coordinate (t123) at (1.8436,0.7970,0.4438);
\coordinate (t124) at (2.0542,0.6767,0.3974);
\coordinate (t125) at (2.1840,0.3174,0.4309);
\coordinate (t126) at (1.6372,0.8873,0.2417);
\coordinate (t127) at (2.2796,0.6998,0.2773);
\coordinate (t128) at (1.6354,0.7836,0.3394);
\coordinate (t129) at (1.8334,0.3420,0.5024);
\coordinate (t130) at (2.1980,0.2715,0.3968);
\coordinate (t131) at (2.0668,0.3528,0.4117);
\coordinate (t132) at (1.8871,0.3451,0.1676);
\coordinate (t133) at (1.9512,0.5861,0.1430);
\coordinate (t134) at (2.3114,0.3994,0.3965);
\coordinate (t135) at (2.1649,0.3128,0.0435);
\coordinate (t136) at (1.6752,0.5497,0.5447);
\coordinate (t137) at (1.8536,0.4192,0.1718);
\coordinate (t138) at (2.0081,0.1512,0.3057);
\coordinate (t139) at (1.9439,0.2945,0.4360);
\coordinate (t140) at (1.7083,0.7005,0.5546);
\coordinate (t141) at (1.7220,0.5803,0.3385);
\coordinate (t142) at (1.8789,0.6277,0.2405);
\coordinate (t143) at (1.9338,0.4143,0.0992);
\coordinate (t144) at (1.8341,0.5443,0.6398);
\coordinate (t145) at (2.1647,0.6237,0.0670);
\coordinate (t146) at (2.3069,0.6776,0.2512);
\coordinate (t147) at (2.2908,0.6543,0.1328);
\coordinate (t148) at (1.6629,0.6961,0.5007);
\coordinate (t149) at (2.3767,0.4098,0.2929);
\coordinate (t150) at (1.7767,0.7407,0.4056);
\coordinate (t151) at (1.6219,0.8202,0.1992);
\coordinate (t152) at (1.7531,0.3383,0.2680);
\coordinate (t153) at (1.8605,0.2902,0.2568);
\coordinate (t154) at (1.7647,0.5774,0.2881);
\coordinate (t155) at (1.9981,0.4387,0.0002);
\coordinate (t156) at (2.3357,0.5048,0.3801);
\coordinate (t157) at (1.9569,0.2717,0.0064);
\coordinate (t158) at (1.9466,0.2785,0.3985);
\coordinate (t159) at (1.6921,0.4603,0.3690);
\coordinate (t160) at (1.6887,0.5218,0.5568);
\coordinate (t161) at (2.0773,0.5393,0.0111);
\coordinate (t162) at (1.8775,0.8150,0.4097);
\coordinate (t163) at (2.1466,0.7233,0.3626);
\coordinate (t164) at (2.2901,0.5962,0.3842);
\coordinate (t165) at (1.9259,0.2948,0.1445);
\coordinate (t166) at (1.8584,0.6319,0.5439);
\coordinate (t167) at (2.1688,0.2418,0.2229);
\coordinate (t168) at (1.9291,0.5551,0.0707);
\coordinate (t169) at (1.9510,0.4028,0.5009);
\coordinate (t170) at (1.9639,0.3179,0.4572);
\coordinate (t171) at (1.8511,0.2951,0.2485);
\coordinate (t172) at (2.4063,0.4378,0.2145);
\coordinate (t173) at (1.6528,0.5898,0.4427);
\coordinate (t174) at (1.9829,0.5849,0.0580);
\coordinate (t175) at (1.9823,0.5307,0.0242);
\coordinate (t176) at (1.8276,0.1626,0.2493);
\coordinate (t177) at (1.9942,0.3788,0.4707);
\coordinate (t178) at (1.7821,0.5894,0.2759);
\coordinate (t179) at (1.9481,0.6630,0.3142);
\coordinate (t180) at (2.3095,0.4821,0.0456);
\coordinate (t181) at (1.7410,0.4514,0.5880);
\coordinate (t182) at (2.1687,0.5392,0.0135);
\coordinate (t183) at (1.8887,0.2893,0.1753);
\coordinate (t184) at (1.8471,0.8280,0.3413);
\coordinate (t185) at (1.6120,0.8262,0.2438);
\coordinate (t186) at (2.2566,0.2567,0.2413);
\coordinate (t187) at (1.7056,0.4854,0.3143);
\coordinate (t188) at (2.1943,0.2524,0.1769);
\coordinate (t189) at (1.9426,0.5308,0.0406);
\coordinate (t190) at (1.9880,0.1411,0.3255);
\coordinate (t191) at (2.3552,0.2942,0.1988);
\coordinate (t192) at (2.0266,0.3844,0.4600);
\coordinate (t193) at (1.9170,0.2746,0.1448);
\coordinate (t194) at (1.9325,0.8639,0.3184);
\coordinate (t195) at (1.6985,0.8052,0.3168);
\coordinate (t196) at (1.7087,0.5571,0.5959);
\coordinate (t197) at (2.2213,0.7278,0.2104);
\coordinate (t198) at (1.8807,0.9277,0.3770);
\coordinate (t199) at (2.3993,0.5197,0.1548);
\coordinate (t200) at (1.8739,0.3939,0.5216);
\coordinate (t201) at (1.6119,0.8278,0.3539);
\coordinate (t202) at (2.3553,0.4807,0.3464);
\coordinate (t203) at (2.0983,0.5874,0.4582);
\coordinate (t204) at (1.6754,0.4961,0.5039);
\coordinate (t205) at (2.0170,0.1370,0.4027);
\coordinate (t206) at (2.3732,0.3331,0.2213);
\coordinate (t207) at (1.8415,0.7097,0.4592);
\coordinate (t208) at (1.8319,0.3320,0.4939);
\coordinate (t209) at (2.2800,0.3083,0.0624);
\coordinate (t210) at (2.1192,0.1571,0.3572);
\coordinate (t211) at (1.8636,0.3517,0.5107);
\coordinate (t212) at (1.9159,0.9566,0.3065);
\coordinate (t213) at (1.7188,0.4274,0.4659);
\coordinate (t214) at (1.8654,0.7618,0.4080);
\coordinate (t215) at (1.9598,0.3734,0.0547);
\coordinate (t216) at (2.1593,0.6974,0.1398);
\coordinate (t217) at (1.8524,0.4203,0.5277);
\coordinate (t218) at (1.8893,0.7941,0.3769);
\coordinate (t219) at (1.6975,0.5284,0.5727);
\coordinate (t220) at (2.3374,0.6377,0.1965);
\coordinate (t221) at (2.1724,0.2719,0.4028);
\coordinate (t222) at (2.1330,0.3390,0.4434);
\coordinate (t223) at (1.9552,0.1453,0.2873);
\coordinate (t224) at (2.4367,0.4512,0.2098);
\coordinate (t225) at (1.9903,0.4339,0.4830);
\coordinate (t226) at (1.8286,0.1572,0.2502);
\coordinate (t227) at (2.3696,0.5881,0.2614);
\coordinate (t228) at (1.8397,0.8590,0.4336);
\coordinate (t229) at (2.3491,0.4766,0.3583);
\coordinate (t230) at (2.4119,0.3487,0.1183);
\coordinate (t231) at (1.8093,0.7230,0.5482);
\coordinate (t232) at (1.9832,0.3057,0.4306);
\coordinate (t233) at (2.0472,0.7083,0.3348);
\coordinate (t234) at (1.7862,0.4603,0.2007);
\coordinate (t235) at (1.9747,0.6792,0.2971);
\coordinate (t236) at (1.8112,0.7543,0.3822);
\coordinate (t237) at (2.0316,0.6783,0.3807);
\coordinate (t238) at (1.9224,0.4621,0.0532);
\coordinate (t239) at (2.2097,0.6117,0.4251);
\coordinate (t240) at (1.8378,0.4532,0.5267);
\coordinate (t241) at (1.8674,0.6113,0.2269);
\coordinate (t242) at (2.1385,0.2230,0.3968);
\coordinate (t243) at (2.2502,0.6770,0.3801);
\coordinate (t244) at (1.9086,0.2099,0.1032);
\coordinate (t245) at (1.7115,0.3779,0.4241);
\coordinate (t246) at (2.2032,0.4357,-0.0230);
\coordinate (t247) at (2.1421,0.4661,0.4873);
\coordinate (t248) at (1.7108,0.7173,0.5221);
\coordinate (t249) at (1.8466,0.9112,0.4034);
\coordinate (t250) at (1.7464,0.4649,0.5250);
\coordinate (t251) at (2.2340,0.2869,0.0944);
\coordinate (t252) at (1.7227,0.7478,0.3497);
\coordinate (t253) at (2.4635,0.4622,0.1080);
\coordinate (t254) at (2.3309,0.6107,0.3386);
\coordinate (t255) at (1.7368,0.6891,0.5857);
\coordinate (t256) at (1.7074,0.5230,0.3587);
\coordinate (t257) at (1.8488,0.2646,0.3464);
\coordinate (t258) at (1.7385,0.4750,0.2514);
\coordinate (t259) at (1.8036,0.7074,0.5744);
\coordinate (t260) at (1.9532,0.5423,0.4815);
\coordinate (t261) at (1.8498,0.3783,0.5226);
\coordinate (t262) at (2.4334,0.4795,0.0665);
\coordinate (t263) at (2.3497,0.6214,0.2097);
\coordinate (t264) at (2.0507,0.7036,0.3498);
\coordinate (t265) at (2.0208,0.2272,0.3848);
\coordinate (t266) at (2.0129,0.6999,0.2394);
\coordinate (t267) at (1.9241,0.5544,0.1234);
\coordinate (t268) at (1.8560,0.8067,0.3474);
\coordinate (t269) at (2.1349,0.2700,0.1367);
\coordinate (t270) at (1.7135,0.7523,0.4416);
\coordinate (t271) at (1.9991,0.5990,0.4409);
\coordinate (t272) at (2.1394,0.3508,-0.0122);
\coordinate (t273) at (2.4663,0.4466,0.1169);
\coordinate (t274) at (1.8899,0.5126,0.5121);
\coordinate (t275) at (2.2665,0.5767,0.4126);
\coordinate (t276) at (1.9488,0.3292,0.4771);
\coordinate (t277) at (1.7503,0.6421,0.6274);
\coordinate (t278) at (2.1525,0.5096,-0.0036);
\coordinate (t279) at (1.6768,0.5141,0.5355);
\coordinate (t280) at (1.7252,0.3867,0.4607);
\coordinate (t281) at (2.1300,0.7365,0.3281);
\coordinate (t282) at (1.6117,0.8293,0.2586);
\coordinate (t283) at (2.3165,0.6338,0.3428);
\coordinate (t284) at (1.7459,0.5222,0.2687);
\coordinate (t285) at (1.6006,0.9092,0.2700);
\coordinate (t286) at (2.1634,0.7169,0.1606);
\coordinate (t287) at (2.3602,0.6017,0.2096);
\coordinate (t288) at (2.0456,0.6160,0.4419);
\coordinate (t289) at (1.8533,0.8929,0.3276);
\coordinate (t290) at (1.6948,0.4379,0.4126);
\coordinate (t291) at (2.1089,0.6288,0.0893);
\coordinate (t292) at (2.0975,0.7305,0.3257);
\coordinate (t293) at (1.8827,0.2935,0.4568);
\coordinate (t294) at (1.9343,0.1905,0.3363);
\coordinate (t295) at (2.4341,0.4559,0.0641);
\coordinate (t296) at (1.9559,0.2770,0.0089);
\coordinate (t297) at (1.7557,0.3510,0.2529);
\coordinate (t298) at (1.9805,0.6212,0.4212);
\coordinate (t299) at (2.2064,0.7328,0.2168);
\coordinate (t300) at (1.8744,0.8049,0.3497);
\coordinate (t301) at (1.9547,0.1904,0.3878);
\coordinate (t302) at (2.4053,0.3370,0.1952);
\coordinate (t303) at (2.0946,0.7411,0.2698);
\coordinate (t304) at (2.2720,0.6421,0.3798);
\coordinate (t305) at (2.3838,0.3622,0.0637);
\coordinate (t306) at (1.6101,0.8211,0.2247);
\coordinate (t307) at (1.9988,0.6804,0.3443);
\coordinate (t308) at (1.9309,0.8500,0.3615);
\coordinate (t309) at (1.9030,0.9139,0.2957);
\coordinate (t310) at (1.7526,0.5270,0.2589);
\coordinate (t311) at (1.9915,0.2569,0.3932);
\coordinate (t312) at (1.8162,0.4096,0.1796);
\coordinate (t313) at (1.7213,0.7694,0.3825);
\coordinate (t314) at (1.8979,0.3069,0.4718);
\coordinate (t315) at (2.0639,0.3330,0.0038);
\coordinate (t316) at (1.7058,0.5208,0.5883);
\coordinate (t317) at (2.2795,0.5674,0.0601);
\coordinate (t318) at (1.7436,0.4600,0.5388);
\coordinate (t319) at (2.2891,0.3844,0.4162);
\coordinate (t320) at (2.3024,0.4711,0.4097);
\coordinate (t321) at (1.9535,0.3731,0.1075);
\coordinate (t322) at (2.3231,0.2481,0.2327);
\coordinate (t323) at (1.8686,0.2687,0.3032);
\coordinate (t324) at (2.0036,0.6172,0.4261);
\coordinate (t325) at (1.9969,0.5848,0.0511);
\coordinate (t326) at (2.0474,0.7097,0.2209);
\coordinate (t327) at (1.7553,0.3302,0.2814);
\coordinate (t328) at (1.7611,0.5610,0.2753);
\coordinate (t329) at (1.7381,0.4558,0.5523);
\coordinate (t330) at (1.8269,0.6275,0.2753);
\coordinate (t331) at (1.9545,0.5796,0.0794);
\coordinate (t332) at (1.6607,0.5833,0.3990);
\coordinate (t333) at (2.3295,0.4974,0.3879);
\coordinate (t334) at (2.0433,0.1825,0.2449);
\coordinate (t335) at (1.7238,0.4685,0.5400);
\coordinate (t336) at (2.1982,0.7392,0.2727);
\coordinate (t337) at (1.7450,0.6899,0.5883);
\coordinate (t338) at (2.2125,0.7173,0.1737);
\coordinate (t339) at (1.9097,0.6210,0.2105);
\coordinate (t340) at (1.7903,0.5662,0.2443);
\coordinate (t341) at (1.7113,0.6223,0.6160);
\coordinate (t342) at (1.7593,0.7347,0.5059);
\coordinate (t343) at (1.6621,0.6376,0.4860);
\coordinate (t344) at (1.6739,0.7623,0.2821);
\coordinate (t345) at (1.7027,0.4479,0.3018);
\coordinate (t346) at (2.3911,0.5077,0.2325);
\coordinate (t347) at (1.7065,0.5903,0.6122);
\coordinate (t348) at (2.2009,0.6507,0.0877);
\coordinate (t349) at (1.8608,0.6649,0.5185);
\coordinate (t350) at (1.7560,0.5162,0.6433);
\coordinate (t351) at (1.7114,0.5065,0.6017);
\coordinate (t352) at (2.0790,0.6123,0.0530);
\coordinate (t353) at (2.2509,0.2133,0.3301);
\coordinate (t354) at (2.2358,0.5358,0.0244);
\coordinate (t355) at (2.3222,0.6583,0.2044);
\coordinate (t356) at (2.4302,0.4533,0.2109);
\coordinate (t357) at (1.8390,0.7265,0.4619);
\coordinate (t358) at (1.8263,0.5025,0.6413);
\coordinate (t359) at (2.0619,0.4583,0.4733);
\coordinate (t360) at (2.1929,0.2449,0.3709);
\coordinate (t361) at (1.9709,0.3262,0.0427);
\coordinate (t362) at (2.2128,0.6992,0.3782);
\coordinate (t363) at (1.9648,0.3426,0.0679);
\coordinate (t364) at (2.1658,0.7119,0.3811);
\coordinate (t365) at (2.2428,0.2481,0.2011);
\coordinate (t366) at (1.9336,0.4158,0.5101);
\coordinate (t367) at (1.9591,0.5420,0.4806);
\coordinate (t368) at (2.1833,0.4264,0.4833);
\coordinate (t369) at (2.2010,0.3931,0.4719);
\coordinate (t370) at (2.0977,0.4751,-0.0077);
\coordinate (t371) at (2.2640,0.6807,0.1443);
\coordinate (t372) at (2.0115,0.3929,0.0002);
\coordinate (t373) at (1.9437,0.9212,0.2729);
\coordinate (t374) at (2.1064,0.6887,0.1380);
\coordinate (t375) at (1.8140,0.6980,0.3883);
\coordinate (t376) at (1.9602,0.6730,0.2719);
\coordinate (t377) at (1.7715,0.4509,0.5495);
\coordinate (t378) at (2.0321,0.7104,0.3074);
\coordinate (t379) at (2.0601,0.1788,0.2653);
\coordinate (t380) at (1.9910,0.3990,0.4760);
\coordinate (t381) at (2.3029,0.6800,0.2954);
\coordinate (t382) at (2.3824,0.3147,0.1497);
\coordinate (t383) at (2.1314,0.3343,-0.0148);
\coordinate (t384) at (2.0053,0.5728,0.0397);
\coordinate (t385) at (2.4079,0.5061,0.1781);
\coordinate (t386) at (2.0206,0.3723,0.0011);
\coordinate (t387) at (2.2185,0.2500,0.1638);
\coordinate (t388) at (1.8871,0.5664,0.5512);
\coordinate (t389) at (1.7051,0.6871,0.3805);
\coordinate (t390) at (2.0642,0.6097,0.4498);
\coordinate (t391) at (1.9497,0.9326,0.2753);
\coordinate (t392) at (1.9047,0.2658,0.3440);
\coordinate (t393) at (1.8795,0.2379,0.2378);
\coordinate (t394) at (1.6525,0.6057,0.4451);
\coordinate (t395) at (1.8831,0.8011,0.4089);
\coordinate (t396) at (2.3546,0.2919,0.2137);
\coordinate (t397) at (1.7098,0.4350,0.2860);
\coordinate (t398) at (1.7094,0.4059,0.2977);
\coordinate (t399) at (2.0965,0.3980,-0.0166);
\coordinate (t400) at (1.8993,0.6002,0.1963);
\coordinate (t401) at (1.9549,0.1855,0.1841);
\coordinate (t402) at (1.8356,0.7284,0.4899);
\coordinate (t403) at (1.6155,0.8170,0.3063);
\coordinate (t404) at (1.7195,0.7036,0.3650);
\coordinate (t405) at (1.8510,0.1606,0.1936);
\coordinate (t406) at (2.2708,0.6998,0.3220);
\coordinate (t407) at (1.9113,0.3439,0.1569);
\coordinate (t408) at (1.8949,1.0177,0.2899);
\coordinate (t409) at (2.0279,0.2733,0.0756);
\coordinate (t410) at (2.2272,0.2507,0.3576);
\coordinate (t411) at (1.8741,0.6589,0.3240);
\coordinate (t412) at (2.0962,0.2615,0.1368);
\coordinate (t413) at (1.8523,0.3175,0.4846);
\coordinate (t414) at (2.3045,0.5280,0.4032);
\coordinate (t415) at (2.0430,0.6090,0.4453);
\coordinate (t416) at (1.8316,0.6204,0.6133);
\coordinate (t417) at (2.1066,0.3376,0.4180);
\coordinate (t418) at (2.1008,0.2392,0.1909);
\coordinate (t419) at (2.2706,0.6062,0.3943);
\coordinate (t420) at (2.1997,0.4848,0.4759);
\coordinate (t421) at (1.7575,0.5808,0.6486);
\coordinate (t422) at (1.8660,0.3186,0.4868);
\coordinate (t423) at (2.1234,0.2085,0.2846);
\coordinate (t424) at (1.8652,0.8717,0.3230);
\coordinate (t425) at (1.5740,0.8922,0.2588);
\coordinate (t426) at (1.9828,0.6381,0.1672);
\coordinate (t427) at (1.6228,0.8836,0.1791);
\coordinate (t428) at (1.9497,0.2369,0.0551);
\coordinate (t429) at (1.8903,0.5661,0.5465);
\coordinate (t430) at (1.6977,0.4985,0.3598);
\coordinate (t431) at (1.8296,0.6092,0.6228);
\coordinate (t432) at (2.2526,0.3048,0.0534);
\coordinate (t433) at (2.3012,0.6556,0.1467);
\coordinate (t434) at (2.3503,0.5098,0.0971);
\coordinate (t435) at (2.0361,0.1737,0.2775);
\coordinate (t436) at (2.2618,0.6643,0.1179);
\coordinate (t437) at (2.3718,0.3684,0.0501);
\coordinate (t438) at (2.3573,0.2965,0.1957);
\coordinate (t439) at (1.8404,0.7180,0.4584);
\coordinate (t440) at (2.0536,0.1439,0.3667);
\coordinate (t441) at (1.6653,0.7198,0.3813);
\coordinate (t442) at (2.1005,0.3551,0.4334);
\coordinate (t443) at (1.7521,0.4301,0.2221);
\coordinate (t444) at (2.1861,0.7202,0.3604);
\coordinate (t445) at (1.9897,0.6597,0.3765);
\coordinate (t446) at (1.9480,0.2719,0.3723);
\coordinate (t447) at (2.1791,0.2385,0.3749);
\coordinate (t448) at (2.1221,0.1742,0.4006);
\coordinate (t449) at (1.6741,0.7110,0.4764);
\coordinate (t450) at (1.8678,0.6654,0.4389);
\coordinate (t451) at (1.6717,0.7080,0.4807);
\coordinate (t452) at (2.1866,0.5987,0.4402);
\coordinate (t453) at (1.9000,0.8893,0.3063);
\coordinate (t454) at (1.9237,0.4301,0.1177);
\coordinate (t455) at (2.1790,0.2999,0.4238);
\coordinate (t456) at (2.0974,0.7418,0.2766);
\coordinate (t457) at (2.2003,0.5846,0.0392);
\coordinate (t458) at (1.6436,0.8685,0.2324);
\coordinate (t459) at (1.7448,0.5909,0.6421);
\coordinate (t460) at (2.3080,0.4666,0.4057);
\coordinate (t461) at (1.7642,0.7538,0.4357);
\coordinate (t462) at (2.2114,0.7342,0.2848);
\coordinate (t463) at (2.0610,0.6372,0.1218);
\coordinate (t464) at (1.9430,0.1723,0.3995);
\coordinate (t465) at (2.2406,0.5557,0.4278);
\coordinate (t466) at (2.0913,0.4011,-0.0137);
\coordinate (t467) at (1.9056,0.4792,0.1285);
\coordinate (t468) at (2.0770,0.7336,0.2924);
\coordinate (t469) at (2.0041,0.5029,0.4762);
\coordinate (t470) at (1.7015,0.3923,0.3241);
\coordinate (t471) at (1.8674,0.8299,0.4011);
\coordinate (t472) at (1.6592,0.6318,0.5126);
\coordinate (t473) at (2.3654,0.4593,0.0336);
\coordinate (t474) at (1.8136,0.6961,0.3868);
\coordinate (t475) at (2.0169,0.3472,0.0085);
\coordinate (t476) at (1.7137,0.4664,0.4639);
\coordinate (t477) at (1.8504,0.1623,0.1890);
\coordinate (t478) at (1.9295,0.2106,0.2804);
\coordinate (t479) at (1.7817,0.4468,0.2032);
\coordinate (t480) at (2.2906,0.2608,0.1803);
\coordinate (t481) at (1.6953,0.4846,0.3890);
\coordinate (t482) at (2.3556,0.5554,0.3418);
\coordinate (t483) at (1.7878,0.4516,0.5257);
\coordinate (t484) at (1.8055,0.7232,0.5483);
\coordinate (t485) at (1.8873,0.2659,0.3628);
\coordinate (t486) at (1.8159,0.8804,0.3857);
\coordinate (t487) at (2.3807,0.3235,0.1180);
\coordinate (t488) at (1.9151,0.5991,0.4545);
\coordinate (t489) at (2.2600,0.5356,0.4295);
\coordinate (t490) at (1.8768,0.3941,0.5212);
\coordinate (t491) at (2.3787,0.5294,0.1645);
\coordinate (t492) at (1.9345,0.4695,0.0353);
\coordinate (t493) at (2.1345,0.3528,0.4582);
\coordinate (t494) at (1.8488,0.9288,0.3472);
\coordinate (t495) at (2.2642,0.3887,0.0196);
\coordinate (t496) at (2.1913,0.6987,0.3907);
\coordinate (t497) at (1.8807,0.6074,0.2118);
\coordinate (t498) at (2.3597,0.3045,0.1327);
\coordinate (t499) at (2.0425,0.6895,0.3722);
\coordinate (t500) at (2.3972,0.3379,0.1142);
\coordinate (t501) at (2.2938,0.5501,0.4091);
\coordinate (t502) at (1.7916,0.6246,0.3274);
\coordinate (t503) at (1.8905,0.6422,0.4207);
\coordinate (t504) at (1.6616,0.5211,0.4996);
\coordinate (t505) at (2.3348,0.3041,0.2872);
\coordinate (t506) at (2.1711,0.5384,0.0130);
\coordinate (t507) at (2.1955,0.3309,0.4350);
\coordinate (t508) at (2.0174,0.3860,0.4626);
\coordinate (t509) at (2.2560,0.3985,0.4401);
\coordinate (t510) at (2.0943,0.6940,0.1457);
\coordinate (t511) at (1.8384,0.5908,0.6100);
\coordinate (t512) at (2.0158,0.3557,0.0062);
\coordinate (t513) at (1.8443,0.8002,0.4422);
\coordinate (t514) at (2.1011,0.7301,0.3294);
\coordinate (t515) at (1.7700,0.7614,0.4287);
\coordinate (t516) at (1.8934,1.0164,0.3216);
\coordinate (t517) at (1.8340,0.2933,0.4475);
\coordinate (t518) at (1.9967,0.4288,0.0011);
\coordinate (t519) at (1.9232,0.5907,0.4580);
\coordinate (t520) at (1.8010,0.4171,0.5171);
\coordinate (t521) at (2.3548,0.4495,0.3414);
\coordinate (t522) at (1.8794,0.2272,0.2491);
\coordinate (t523) at (1.7660,0.3240,0.4293);
\coordinate (t524) at (2.2985,0.2328,0.2542);
\coordinate (t525) at (1.8529,0.5706,0.5891);
\coordinate (t526) at (1.8304,0.4783,0.6289);
\coordinate (t527) at (1.6426,0.7938,0.3931);
\coordinate (t528) at (2.2800,0.2513,0.2244);
\coordinate (t529) at (2.1196,0.3888,-0.0193);
\coordinate (t530) at (1.8066,0.2983,0.2722);
\coordinate (t531) at (2.0901,0.7303,0.2172);
\coordinate (t532) at (1.6075,0.8324,0.1959);
\coordinate (t533) at (1.8908,0.3456,0.1647);
\coordinate (t534) at (2.3251,0.6297,0.1467);
\coordinate (t535) at (2.1829,0.5881,0.4441);
\coordinate (t536) at (1.8429,0.6351,0.5701);
\coordinate (t537) at (2.3748,0.3674,0.2762);
\coordinate (t538) at (2.0138,0.7059,0.2685);
\coordinate (t539) at (1.8340,0.8357,0.3458);
\coordinate (t540) at (2.3185,0.5311,0.3947);
\coordinate (t541) at (1.7438,0.5968,0.6404);
\coordinate (t542) at (1.7362,0.3342,0.3976);
\coordinate (t543) at (2.3099,0.5326,0.0630);
\coordinate (t544) at (1.6682,0.4980,0.4693);
\coordinate (t545) at (2.4404,0.4768,0.0731);
\coordinate (t546) at (2.1977,0.3786,0.4668);
\coordinate (t547) at (2.4049,0.4210,0.2185);
\coordinate (t548) at (1.6717,0.5838,0.3852);
\coordinate (t549) at (1.9266,0.5038,0.5022);
\coordinate (t550) at (1.7174,0.4433,0.4627);
\coordinate (t551) at (1.9688,0.1124,0.4085);
\coordinate (t552) at (1.8452,0.7955,0.4407);
\coordinate (t553) at (2.2632,0.3801,0.0249);
\coordinate (t554) at (1.6619,0.5165,0.4365);
\coordinate (t555) at (2.0573,0.5645,0.4626);
\coordinate (t556) at (1.6119,0.8437,0.3472);
\coordinate (t557) at (1.7254,0.7538,0.3585);
\coordinate (t558) at (2.0694,0.2899,-0.0021);
\coordinate (t559) at (1.8744,0.1761,0.2784);
\coordinate (t560) at (1.7882,0.3807,0.5024);
\coordinate (t561) at (1.6035,0.9124,0.1743);
\coordinate (t562) at (1.9454,0.3032,0.1389);
\coordinate (t563) at (1.8866,0.5693,0.5507);
\coordinate (t564) at (1.6251,0.8874,0.2837);
\coordinate (t565) at (2.1209,0.5927,0.4569);
\coordinate (t566) at (1.7873,0.5493,0.2390);
\coordinate (t567) at (1.8208,0.6252,0.2782);
\coordinate (t568) at (2.2392,0.6415,0.4009);
\coordinate (t569) at (2.3520,0.4357,0.3343);
\coordinate (t570) at (1.5761,0.9473,0.2437);
\coordinate (t571) at (2.0164,0.2793,-0.0009);
\coordinate (t572) at (1.7256,0.5479,0.3277);
\coordinate (t573) at (1.9576,0.1173,0.4089);
\coordinate (t574) at (2.3065,0.2288,0.2679);
\coordinate (t575) at (2.2070,0.5564,0.0247);
\coordinate (t576) at (1.7108,0.5666,0.6103);
\coordinate (t577) at (1.8737,0.6499,0.4889);
\coordinate (t578) at (1.7455,0.5750,0.6446);
\coordinate (t579) at (1.7213,0.7257,0.5099);
\coordinate (t580) at (2.1970,0.3414,0.4414);
\coordinate (t581) at (2.0260,0.6871,0.3603);
\coordinate (t582) at (1.9538,0.3774,0.0871);
\coordinate (t583) at (2.0033,0.2690,0.0573);
\coordinate (t584) at (1.6569,0.5357,0.4472);
\coordinate (t585) at (1.7509,0.6229,0.6354);
\coordinate (t586) at (2.0708,0.1919,0.2658);
\coordinate (t587) at (2.3961,0.4029,0.0442);
\coordinate (t588) at (2.0384,0.1646,0.2884);
\coordinate (t589) at (2.2040,0.5748,0.0342);
\coordinate (t590) at (2.2555,0.6242,0.0752);
\coordinate (t591) at (1.9111,0.1642,0.3355);
\coordinate (t592) at (1.6967,0.5032,0.3780);
\coordinate (t593) at (2.1261,0.3297,0.4280);
\coordinate (t594) at (2.1140,0.2724,0.1210);
\coordinate (t595) at (2.0919,0.3352,0.4021);
\coordinate (t596) at (1.9658,0.3180,0.4566);
\coordinate (t597) at (2.0381,0.4107,0.4581);
\coordinate (t598) at (1.7773,0.3918,0.2029);
\coordinate (t599) at (1.8703,0.7737,0.4087);
\coordinate (t600) at (1.7749,0.6760,0.3597);
\coordinate (t601) at (2.1944,0.2522,0.2107);
\coordinate (t602) at (2.3544,0.3407,0.2900);
\coordinate (t603) at (1.9892,0.6792,0.2260);
\coordinate (t604) at (1.6385,0.7633,0.3241);
\coordinate (t605) at (1.9504,0.6059,0.1555);
\coordinate (t606) at (1.5762,0.9534,0.2332);
\coordinate (t607) at (1.6054,0.8445,0.2606);
\coordinate (t608) at (1.8752,0.5425,0.1734);
\coordinate (t609) at (1.9906,0.6749,0.3468);
\coordinate (t610) at (1.8927,1.0148,0.3279);
\coordinate (t611) at (1.9801,0.1123,0.3979);
\coordinate (t612) at (2.3280,0.2965,0.2939);
\coordinate (t613) at (2.1689,0.3715,0.4700);
\coordinate (t614) at (2.0600,0.7274,0.2891);
\coordinate (t615) at (1.7123,0.5001,0.6019);
\coordinate (t616) at (1.6651,0.5301,0.5217);
\coordinate (t617) at (2.2595,0.5770,0.4144);
\coordinate (t618) at (2.0759,0.7210,0.3325);
\coordinate (t619) at (1.8820,0.5857,0.1963);
\coordinate (t620) at (2.4625,0.4985,0.1463);
\coordinate (t621) at (1.8040,0.8225,0.3789);
\coordinate (t622) at (2.1458,0.2549,0.1769);
\coordinate (t623) at (2.0688,0.2762,0.0223);
\coordinate (t624) at (2.2159,0.2789,0.1118);
\coordinate (t625) at (1.9478,0.2253,0.2876);
\coordinate (t626) at (2.0326,0.6124,0.0743);
\coordinate (t627) at (2.0337,0.6881,0.1908);
\coordinate (t628) at (2.3818,0.4878,0.0478);
\coordinate (t629) at (1.8637,0.3040,0.2260);
\coordinate (t630) at (2.1620,0.5301,0.0071);
\coordinate (t631) at (1.9715,0.2146,0.3670);
\coordinate (t632) at (1.8669,0.3079,0.2029);
\coordinate (t633) at (1.6220,0.7924,0.3436);
\coordinate (t634) at (2.1228,0.2768,0.1154);
\coordinate (t635) at (1.6326,0.7706,0.3700);
\coordinate (t636) at (2.1019,0.4066,-0.0148);
\coordinate (t637) at (1.8854,0.6416,0.4784);
\coordinate (t638) at (1.8800,0.1878,0.1412);
\coordinate (t639) at (1.7581,0.6035,0.6437);
\coordinate (t640) at (1.8313,0.8952,0.4066);
\coordinate (t641) at (1.8476,0.8468,0.3352);
\coordinate (t642) at (2.2962,0.6002,0.0823);
\coordinate (t643) at (2.3893,0.3813,0.0522);
\coordinate (t644) at (1.7484,0.3217,0.3899);
\coordinate (t645) at (1.7681,0.3062,0.3283);
\coordinate (t646) at (1.7007,0.6950,0.5576);
\coordinate (t647) at (2.4036,0.5290,0.1231);
\coordinate (t648) at (1.6804,0.6671,0.4013);
\coordinate (t649) at (2.3405,0.2879,0.1543);
\coordinate (t650) at (1.7030,0.5238,0.3667);
\coordinate (t651) at (2.3472,0.4505,0.3635);
\coordinate (t652) at (2.2022,0.3466,-0.0181);
\coordinate (t653) at (2.0256,0.4981,0.0094);
\coordinate (t654) at (1.8956,1.0092,0.2780);
\coordinate (t655) at (2.4656,0.4102,0.1406);
\coordinate (t656) at (2.0954,0.6819,0.1370);
\coordinate (t657) at (1.9644,0.2488,0.3688);
\coordinate (t658) at (2.2270,0.6356,0.4070);
\coordinate (t659) at (1.6594,0.7994,0.3998);
\coordinate (t660) at (2.3359,0.6264,0.3142);
\coordinate (t661) at (2.1951,0.5263,0.4399);
\coordinate (t662) at (1.8070,0.7418,0.4998);
\coordinate (t663) at (1.6759,0.5034,0.4229);
\coordinate (t664) at (1.7923,0.7235,0.3943);
\coordinate (t665) at (1.8558,0.7486,0.4234);
\coordinate (t666) at (1.5890,0.8651,0.2728);
\coordinate (t667) at (2.3639,0.6040,0.2543);
\coordinate (t668) at (2.1344,0.7350,0.1997);
\coordinate (t669) at (2.0727,0.4727,-0.0069);
\coordinate (t670) at (1.9551,0.1843,0.3958);
\coordinate (t671) at (2.0167,0.6974,0.3246);
\coordinate (t672) at (2.0425,0.1524,0.3256);
\coordinate (t673) at (2.2711,0.2965,0.0927);
\coordinate (t674) at (2.2192,0.1924,0.3163);
\coordinate (t675) at (1.9213,0.2883,0.0490);
\coordinate (t676) at (2.0989,0.5480,0.4638);
\coordinate (t677) at (1.8575,0.8450,0.4266);
\coordinate (t678) at (2.0233,0.5360,0.0158);
\coordinate (t679) at (2.3471,0.4842,0.0725);
\coordinate (t680) at (1.9098,0.9974,0.2973);
\coordinate (t681) at (2.0302,0.5021,0.0092);
\coordinate (t682) at (2.3934,0.4967,0.2289);
\coordinate (t683) at (2.3245,0.3344,0.0550);
\coordinate (t684) at (2.3698,0.4625,0.3214);
\coordinate (t685) at (1.9093,0.3925,0.1529);
\coordinate (t686) at (2.3004,0.5438,0.0643);
\coordinate (t687) at (1.7928,0.5057,0.6505);
\coordinate (t688) at (1.8602,0.6601,0.5270);
\coordinate (t689) at (2.3049,0.6770,0.3032);
\coordinate (t690) at (1.9920,0.2538,0.0423);
\coordinate (t691) at (2.4062,0.3939,0.0558);
\coordinate (t692) at (1.6961,0.7832,0.4091);
\coordinate (t693) at (2.1366,0.2442,0.3772);
\coordinate (t694) at (2.3806,0.4055,0.0365);
\coordinate (t695) at (2.3699,0.4440,0.0301);
\coordinate (t696) at (1.9066,0.9508,0.2768);
\coordinate (t697) at (1.9020,0.2423,0.0490);
\coordinate (t698) at (2.3530,0.2917,0.1987);
\coordinate (t699) at (2.0894,0.5412,0.4657);
\coordinate (t700) at (1.8084,0.8673,0.4015);
\coordinate (t701) at (1.8610,0.5753,0.5711);
\coordinate (t702) at (2.3813,0.4118,0.2884);
\coordinate (t703) at (1.8589,0.2263,0.1836);
\coordinate (t704) at (2.3553,0.5881,0.1638);
\coordinate (t705) at (2.1370,0.1732,0.4049);
\coordinate (t706) at (1.9607,0.3539,0.1364);
\coordinate (t707) at (2.0261,0.3581,0.0019);
\coordinate (t708) at (2.3061,0.5496,0.0719);
\coordinate (t709) at (1.8632,0.6576,0.3175);
\coordinate (t710) at (1.9372,0.5659,0.1276);
\coordinate (t711) at (2.0295,0.2624,0.3999);
\coordinate (t712) at (1.9333,0.4404,0.0516);
\coordinate (t713) at (1.9103,0.1495,0.3195);
\coordinate (t714) at (1.9063,0.6579,0.3556);
\coordinate (t715) at (2.1936,0.6093,0.4351);
\coordinate (t716) at (1.6821,0.4979,0.5264);
\coordinate (t717) at (1.9100,0.2469,0.1188);
\coordinate (t718) at (2.3591,0.2980,0.2255);
\coordinate (t719) at (1.8603,0.4157,0.5276);
\coordinate (t720) at (2.1271,0.5778,0.0279);
\coordinate (t721) at (2.0843,0.3541,-0.0077);
\coordinate (t722) at (1.9050,0.5136,0.5036);
\coordinate (t723) at (2.1395,0.4384,-0.0198);
\coordinate (t724) at (1.5755,0.9227,0.2699);
\coordinate (t725) at (1.8052,0.3300,0.4836);
\coordinate (t726) at (1.8717,0.5109,0.1608);
\coordinate (t727) at (1.7685,0.3971,0.2085);
\coordinate (t728) at (1.9498,0.4194,0.5057);
\coordinate (t729) at (1.9934,0.1899,0.1966);
\coordinate (t730) at (2.4132,0.4630,0.2080);
\coordinate (t731) at (1.9202,0.2744,0.1190);
\coordinate (t732) at (2.1932,0.5063,0.4632);
\coordinate (t733) at (1.8495,0.2167,0.2261);
\coordinate (t734) at (1.6530,0.8658,0.2876);
\coordinate (t735) at (1.8731,0.5110,0.5590);
\coordinate (t736) at (2.3124,0.4895,0.0500);
\coordinate (t737) at (1.9651,0.1199,0.4126);
\coordinate (t738) at (2.0667,0.1475,0.3578);
\coordinate (t739) at (2.0060,0.5672,0.4598);
\coordinate (t740) at (2.3704,0.4350,0.0291);
\coordinate (t741) at (1.6628,0.6098,0.5394);
\coordinate (t742) at (1.9447,0.1935,0.3698);
\coordinate (t743) at (2.3235,0.4792,0.0603);
\coordinate (t744) at (2.2255,0.1900,0.3265);
\coordinate (t745) at (1.7376,0.5572,0.3159);
\coordinate (t746) at (2.1905,0.5596,0.4369);
\coordinate (t747) at (1.9409,0.2633,0.3403);
\coordinate (t748) at (2.0018,0.1939,0.2055);
\coordinate (t749) at (1.9765,0.1499,0.4190);
\coordinate (t750) at (1.8184,0.8058,0.4531);
\coordinate (t751) at (1.6636,0.6506,0.4789);
\coordinate (t752) at (2.1178,0.6260,0.0778);
\coordinate (t753) at (2.0625,0.7250,0.3055);
\coordinate (t754) at (2.0886,0.4996,-0.0017);
\coordinate (t755) at (1.9652,0.3358,0.0771);
\coordinate (t756) at (1.9688,0.6380,0.4037);
\coordinate (t757) at (2.0872,0.5499,0.4650);
\coordinate (t758) at (1.8624,0.8607,0.4159);
\coordinate (t759) at (1.6958,0.4118,0.3260);
\coordinate (t760) at (1.8333,0.6180,0.2580);
\coordinate (t761) at (2.1399,0.4263,0.4945);
\coordinate (t762) at (1.9485,0.2388,0.3249);
\coordinate (t763) at (2.2102,0.4565,-0.0153);
\coordinate (t764) at (1.8286,0.6645,0.5990);
\coordinate (t765) at (2.0971,0.6117,0.4538);
\coordinate (t766) at (2.0299,0.6183,0.4351);
\coordinate (t767) at (2.2534,0.6135,0.4011);
\coordinate (t768) at (2.3941,0.5077,0.0696);
\coordinate (t769) at (2.1375,0.5960,0.0380);
\coordinate (t770) at (2.3150,0.6648,0.1968);
\coordinate (t771) at (1.6931,0.7861,0.4078);
\coordinate (t772) at (2.0989,0.5963,0.4573);
\coordinate (t773) at (1.7848,0.3372,0.2458);
\coordinate (t774) at (1.8017,0.4496,0.5518);
\coordinate (t775) at (1.7084,0.4068,0.4411);
\coordinate (t776) at (1.8599,0.1924,0.2675);
\coordinate (t777) at (2.3616,0.4539,0.3330);
\coordinate (t778) at (2.1711,0.5869,0.0350);
\coordinate (t779) at (1.5893,0.8899,0.3005);
\coordinate (t780) at (2.3886,0.3228,0.1361);
\coordinate (t781) at (2.1958,0.3293,0.4346);
\coordinate (t782) at (1.7367,0.6972,0.5762);
\coordinate (t783) at (1.9252,0.9901,0.2633);
\coordinate (t784) at (1.7115,0.5814,0.3458);
\coordinate (t785) at (2.2639,0.6550,0.1117);
\coordinate (t786) at (2.1932,0.3436,-0.0206);
\coordinate (t787) at (2.1669,0.3558,0.4607);
\coordinate (t788) at (1.8120,0.7836,0.4614);
\coordinate (t789) at (1.6506,0.7513,0.3578);
\coordinate (t790) at (1.7175,0.3601,0.3725);
\coordinate (t791) at (1.9047,0.4889,0.1210);
\coordinate (t792) at (1.6396,0.8805,0.2685);
\coordinate (t793) at (1.6111,0.9405,0.2013);
\coordinate (t794) at (2.0411,0.3534,-0.0014);
\coordinate (t795) at (2.0239,0.1984,0.1899);
\coordinate (t796) at (1.7180,0.5510,0.6172);
\coordinate (t797) at (2.0360,0.2792,0.0023);
\coordinate (t798) at (2.0726,0.5894,0.4576);
\coordinate (t799) at (2.2973,0.6008,0.3790);
\coordinate (t800) at (2.2065,0.4592,-0.0156);
\coordinate (t801) at (2.1571,0.2375,0.2270);
\coordinate (t802) at (2.1885,0.5837,0.4417);
\coordinate (t803) at (1.8831,0.4497,0.1585);
\coordinate (t804) at (1.9761,0.4644,0.4962);
\coordinate (t805) at (2.3528,0.4582,0.3504);
\coordinate (t806) at (1.9889,0.4419,0.0030);
\coordinate (t807) at (2.4466,0.4021,0.2009);
\coordinate (t808) at (2.3590,0.3218,0.2608);
\coordinate (t809) at (1.8931,0.3620,0.5174);
\coordinate (t810) at (1.8029,0.8443,0.3887);
\coordinate (t811) at (2.4236,0.5288,0.1124);
\coordinate (t812) at (2.1638,0.4826,0.4800);
\coordinate (t813) at (2.2027,0.2895,0.0612);
\coordinate (t814) at (1.8629,0.9534,0.3328);
\coordinate (t815) at (2.2995,0.6462,0.1333);
\coordinate (t816) at (2.2917,0.2388,0.2418);
\coordinate (t817) at (2.4129,0.3772,0.0761);
\coordinate (t818) at (1.7445,0.4287,0.4912);
\coordinate (t819) at (1.8283,0.5320,0.6463);
\coordinate (t820) at (1.9490,0.6667,0.2805);
\coordinate (t821) at (1.9706,0.4017,0.0228);
\coordinate (t822) at (2.2328,0.5048,0.4551);
\coordinate (t823) at (1.9620,0.3498,0.1361);
\coordinate (t824) at (1.8836,0.2483,0.1702);
\coordinate (t825) at (2.1148,0.2201,0.2462);
\coordinate (t826) at (1.9054,0.4830,0.1264);
\coordinate (t827) at (2.2460,0.1982,0.3282);
\coordinate (t828) at (1.9409,0.2323,0.2804);
\coordinate (t829) at (2.3069,0.5130,0.4001);
\coordinate (t830) at (1.7964,0.7936,0.4544);
\coordinate (t831) at (1.9343,0.6609,0.2937);
\coordinate (t832) at (1.8438,0.1510,0.2156);
\coordinate (t833) at (2.2244,0.5172,0.0133);
\coordinate (t834) at (2.2165,0.2437,0.2500);
\coordinate (t835) at (1.6963,0.7182,0.5024);
\coordinate (t836) at (2.2058,0.4504,-0.0192);
\coordinate (t837) at (1.8981,0.2658,0.1593);
\coordinate (t838) at (1.9379,0.2918,0.1201);
\coordinate (t839) at (2.4604,0.4052,0.1725);
\coordinate (t840) at (1.8754,0.2732,0.4089);
\coordinate (t841) at (1.5886,0.8392,0.3040);
\coordinate (t842) at (1.8702,0.9517,0.3167);
\coordinate (t843) at (2.1035,0.3188,0.3946);
\coordinate (t844) at (1.7534,0.3306,0.2836);
\coordinate (t845) at (2.3172,0.2363,0.2583);
\coordinate (t846) at (1.8043,0.5508,0.2222);
\coordinate (t847) at (2.1706,0.5270,0.4411);
\coordinate (t848) at (1.9116,0.2774,0.0752);
\coordinate (t849) at (2.0120,0.6966,0.2322);
\coordinate (t850) at (1.8623,0.6703,0.4290);
\coordinate (t851) at (1.8262,0.1833,0.2122);
\coordinate (t852) at (2.1385,0.4210,-0.0232);
\coordinate (t853) at (2.2257,0.6437,0.4067);
\coordinate (t854) at (1.9795,0.6758,0.3270);
\coordinate (t855) at (2.4266,0.3666,0.1092);
\coordinate (t856) at (1.9115,0.3284,0.1562);
\coordinate (t857) at (1.8594,0.3278,0.4944);
\coordinate (t858) at (2.0256,0.6334,0.4201);
\coordinate (t859) at (1.7532,0.6629,0.6153);
\coordinate (t860) at (2.0430,0.2534,0.1279);
\coordinate (t861) at (1.6424,0.8686,0.2294);
\coordinate (t862) at (1.7005,0.4818,0.5179);
\coordinate (t863) at (1.9292,0.5115,0.0444);
\coordinate (t864) at (1.8054,0.7890,0.3773);
\coordinate (t865) at (2.1845,0.2589,0.1377);
\coordinate (t866) at (2.3887,0.3583,0.2172);
\coordinate (t867) at (1.8421,0.6385,0.2792);
\coordinate (t868) at (2.4464,0.5068,0.1728);
\coordinate (t869) at (1.7344,0.4440,0.4813);
\coordinate (t870) at (1.7833,0.6638,0.3520);
\coordinate (t871) at (2.2628,0.7109,0.2772);
\coordinate (t872) at (2.1536,0.3109,0.0482);
\coordinate (t873) at (1.9161,1.0047,0.2700);
\coordinate (t874) at (1.9914,0.5485,0.0280);
\coordinate (t875) at (1.6855,0.7074,0.5159);
\coordinate (t876) at (2.2191,0.3006,0.4196);
\coordinate (t877) at (2.2907,0.2206,0.2822);
\coordinate (t878) at (1.6588,0.8437,0.2518);
\coordinate (t879) at (1.7541,0.5233,0.2535);
\coordinate (t880) at (1.9133,0.2668,0.1446);
\coordinate (t881) at (2.2441,0.3261,0.0317);
\coordinate (t882) at (2.3105,0.5039,0.0519);
\coordinate (t883) at (1.8806,0.3639,0.5180);
\coordinate (t884) at (1.8588,0.1760,0.1602);
\coordinate (t885) at (1.8427,0.5664,0.2042);
\coordinate (t886) at (2.3331,0.5132,0.3821);
\coordinate (t887) at (1.8494,0.7634,0.3718);
\coordinate (t888) at (2.2643,0.2537,0.1838);
\coordinate (t889) at (1.7009,0.6076,0.3576);
\coordinate (t890) at (2.1968,0.5397,0.4342);
\coordinate (t891) at (1.9883,0.6403,0.4007);
\coordinate (t892) at (2.1138,0.4802,0.4665);
\coordinate (t893) at (1.8060,0.3967,0.1864);
\coordinate (t894) at (1.8045,0.5727,0.6545);
\coordinate (t895) at (2.0830,0.3407,-0.0009);
\coordinate (t896) at (1.9924,0.4318,0.0029);
\coordinate (t897) at (1.7255,0.3509,0.3265);
\coordinate (t898) at (2.0107,0.1990,0.3853);
\coordinate (t899) at (1.7667,0.3287,0.4449);
\coordinate (t900) at (2.0813,0.2336,0.1945);
\coordinate (t901) at (1.9741,0.5917,0.4556);
\coordinate (t902) at (2.0672,0.7293,0.2947);
\coordinate (t903) at (1.8496,0.3299,0.4951);
\coordinate (t904) at (1.8619,0.3074,0.2248);
\coordinate (t905) at (2.0350,0.3930,-0.0089);
\coordinate (t906) at (1.8446,0.3388,0.2082);
\coordinate (t907) at (1.7129,0.3817,0.4317);
\coordinate (t908) at (1.9211,0.9845,0.2836);
\coordinate (t909) at (2.0720,0.5711,0.4620);
\coordinate (t910) at (2.2985,0.2540,0.3078);
\coordinate (t911) at (1.8247,0.6640,0.3575);
\coordinate (t912) at (1.7260,0.7322,0.4930);
\coordinate (t913) at (2.3255,0.6314,0.1500);
\coordinate (t914) at (2.0242,0.6461,0.1390);
\coordinate (t915) at (2.1794,0.7374,0.3121);
\coordinate (t916) at (1.8231,0.2895,0.4319);
\coordinate (t917) at (2.1546,0.6590,0.0933);
\coordinate (t918) at (2.0032,0.6008,0.4397);
\coordinate (t919) at (1.6137,0.8121,0.2067);
\coordinate (t920) at (2.1772,0.5461,0.0167);
\coordinate (t921) at (1.8742,0.2149,0.1460);
\coordinate (t922) at (2.2102,0.7355,0.2746);
\coordinate (t923) at (1.6024,0.8558,0.2251);
\coordinate (t924) at (1.7448,0.5770,0.3238);
\coordinate (t925) at (1.9036,0.6303,0.2228);
\coordinate (t926) at (1.9081,0.5261,0.1403);
\coordinate (t927) at (1.9553,0.3292,0.1443);
\coordinate (t928) at (2.3423,0.4628,0.0487);
\coordinate (t929) at (2.1142,0.3269,0.4136);
\coordinate (t930) at (1.6036,0.9021,0.1741);
\coordinate (t931) at (2.4326,0.4941,0.1921);
\coordinate (t932) at (1.9050,0.1357,0.3404);
\coordinate (t933) at (1.8043,0.6200,0.2946);
\coordinate (t934) at (2.1365,0.3663,0.4731);
\coordinate (t935) at (1.9778,0.2260,0.3715);
\coordinate (t936) at (1.7784,0.7005,0.5826);
\coordinate (t937) at (2.3800,0.3124,0.1552);
\coordinate (t938) at (2.4602,0.4055,0.1737);
\coordinate (t939) at (2.2270,0.5208,0.4419);
\coordinate (t940) at (2.0731,0.2772,0.0903);
\coordinate (t941) at (2.1359,0.2608,0.1579);
\coordinate (t942) at (1.8512,0.6869,0.5125);
\coordinate (t943) at (2.1518,0.3112,0.0379);
\coordinate (t944) at (1.8847,0.8310,0.3342);
\coordinate (t945) at (2.2246,0.2859,0.0765);
\coordinate (t946) at (2.2626,0.7082,0.2049);
\coordinate (t947) at (2.0308,0.1399,0.3525);
\coordinate (t948) at (1.9201,0.4754,0.0527);
\coordinate (t949) at (2.0850,0.5672,0.0236);
\coordinate (t950) at (2.4566,0.4259,0.1959);
\coordinate (t951) at (2.2213,0.7321,0.2562);
\coordinate (t952) at (2.0013,0.2359,0.1503);
\coordinate (t953) at (1.9736,0.2590,0.3837);
\coordinate (t954) at (2.1954,0.2545,0.1449);
\coordinate (t955) at (2.1979,0.7378,0.2848);
\coordinate (t956) at (1.9901,0.3244,0.4467);
\coordinate (t957) at (1.9869,0.3417,0.4616);
\coordinate (t958) at (2.3136,0.6705,0.2286);
\coordinate (t959) at (1.7992,0.7179,0.5582);
\coordinate (t960) at (1.9350,0.1178,0.3566);
\coordinate (t961) at (2.2021,0.5639,0.0274);
\coordinate (t962) at (2.0252,0.4359,-0.0023);
\coordinate (t963) at (1.9790,0.2603,0.0829);
\coordinate (t964) at (1.8467,0.6964,0.5529);
\coordinate (t965) at (1.8572,0.1773,0.1563);
\coordinate (t966) at (2.3713,0.5791,0.2161);
\coordinate (t967) at (2.3550,0.2957,0.2656);
\coordinate (t968) at (1.9310,0.1280,0.3942);
\coordinate (t969) at (1.7437,0.3253,0.3209);
\coordinate (t970) at (2.0658,0.1787,0.2766);
\coordinate (t971) at (1.9085,0.2456,0.1126);
\coordinate (t972) at (1.9649,0.3958,0.4960);
\coordinate (t973) at (2.4681,0.4363,0.1236);
\coordinate (t974) at (1.8025,0.4775,0.1883);
\coordinate (t975) at (2.0312,0.2605,0.3984);
\coordinate (t976) at (2.3825,0.4502,0.2871);
\coordinate (t977) at (1.7143,0.5208,0.6074);
\coordinate (t978) at (2.4064,0.3314,0.1683);
\coordinate (t979) at (1.6680,0.6253,0.4124);
\coordinate (t980) at (1.8565,0.1943,0.1532);
\coordinate (t981) at (1.7966,0.5187,0.6579);
\coordinate (t982) at (1.7789,0.5499,0.6588);
\coordinate (t983) at (2.3953,0.4520,0.2292);
\coordinate (t984) at (1.8557,0.4689,0.5955);
\coordinate (t985) at (1.8739,0.6589,0.3230);
\coordinate (t986) at (1.9650,0.3830,0.4966);
\coordinate (t987) at (2.2489,0.7057,0.1736);
\coordinate (t988) at (1.8053,0.4261,0.1823);
\coordinate (t989) at (2.2836,0.5431,0.4151);
\coordinate (t990) at (2.0231,0.2651,0.0203);
\coordinate (t991) at (1.8617,0.8428,0.3312);
\coordinate (t992) at (1.6606,0.5424,0.4109);
\coordinate (t993) at (1.7966,0.5072,0.6514);
\coordinate (t994) at (2.0407,0.5516,0.4621);
\coordinate (t995) at (1.8561,0.2978,0.4635);
\coordinate (t996) at (2.1771,0.6593,0.4213);
\coordinate (t997) at (2.1476,0.2326,0.2340);
\coordinate (t998) at (1.7953,0.2884,0.3545);
\coordinate (t999) at (2.3869,0.5357,0.2350);

% % Correspondence indices
% \def\correspondences{{521,737,740,660,411,678,626,513,859,136,811,76,636,973,938,899,280,883,761,319,549,174,371,527,210,235,101,986,902,947,346,139,621,499,370,198,687,584,901,59,328,96,312,974,299,277,924,601,439,837}

